The de Haas van Alphen effect near a quantum critical end point in Sr_3Ru_2O_7

Highly correlated electron materials are systems in which many new states of matter can emerge. A particular situation which favours the formation of exotic phases of the electron liquid in complex materials is that where a quantum critical point (QCP) is present the phase diagram. Neighbouring regions in parameter space reveal unusual physical properties, described as non-Fermi liquid behaviour. One of the important problems in quantum criticality is to find out how the Fermi surface (FS) of a material evolves near a QCP. The traditional method for studying the FS of materials is the de Haas van Alphen effect (dHvA). A quantum critical end point (QCEP) has been reported in the highly correlated metal Sr3Ru2O7, which is tuned using a magnetic field high enough to perform the dHvA experiment. It moreover features a new emergent phase in the vicinity of the QCEP, a nematic type of electron ordering. The subject of this thesis is the study of the FS of Sr3Ru2O7 using the dHvA effect. Three aspects were explored. The first was the determination of the FS at fields both above and below that where the QCEP arises. The second was the search for quantum oscillations inside the nematic phase. The third was a reinvestigation of the behaviour of the quasiparticle effective masses near the FS. A complete robust model for the FS of Sr3Ru2O7 at zero fields was determined. Moreover, the new measurements of the quasiparticle masses revealed that no mass enhancements exist anywhere around the QCEP. Finally, we report dHvA oscillations inside the nematic phase, which suggests that the carriers consist of Landau quasiparticles.

==> Abstract.tex <==
 

Highly correlated electron materials are systems in which many new states of matter can emerge. A particular situation which favours the formation of exotic phases of the electron liquid in complex materials is that where a quantum critical point (QCP) is present the phase diagram. Neighbouring regions in parameter space reveal unusual physical properties, described as non-Fermi liquid behaviour. 

One of the important problems in quantum criticality is to find out how the Fermi surface (FS) of a material evolves near a QCP. The traditional method for studying the FS of materials is the de Haas van Alphen effect (dHvA). A quantum critical end point (QCEP) has been reported in the highly correlated metal \TTS, which is tuned using a magnetic field high enough to perform the dHvA experiment. It moreover features a new emergent phase in the vicinity of the QCEP, a nematic type of electron ordering. 

The subject of this thesis is the study of the FS of \TTS\ using the dHvA effect. Three aspects were explored. The first was the determination of the FS at fields both above and below that where the QCEP arises. The second was the search for quantum oscillations inside the nematic phase. The third was a reinvestigation of the behaviour of the quasiparticle effective masses near the FS. 

In collaboration with angle resolved photoemission spectroscopy experimentalists, a complete robust model for the FS of \TTS\ at zero fields was determined. Moreover, the new measurements of the quasiparticle masses revealed that no mass enhancements exist anywhere around the QCEP, in contradiction with previous specific heat data and measurements of the $A$ coefficient of the power law of the resistivity. Finally, we report dHvA oscillations inside the nematic phase, and the temperature dependence of their amplitude suggests strongly that the carriers consist of Landau quasiparticles. 



==> Acknowledgements.tex <==
 


I would like first to thank my supervisor, Prof. Andrew Mackenzie, for guiding me through this undertaking. He let me carry out this project in my own way, putting up with my stubbornness and pushed me to lay my work onto firm scientific grounds. He enabled me to travel throughout this Ph. D. , and to perform experiments in one of the most famous and historic laboratories, the Cavendish Laboratory in Cambridge. 

I also wish to thank the ones who taught me the secrets of cryogenics and the dHvA experiments themselves, Dr. Rodolfo Borzi, Dr. Robin Perry and Dr. Philipp Gegenwart. I thank Dr. Chris Hooley for all the encouragement he gave me, and for all the theoretical insights over sometimes very basic physics. I am grateful to Dr. Santiago Grigera and Dr. Andrew Green for helpful discussions and the stimulation interactions between theorists and experimentalists, and making life within our research group very dynamic. 

I thank my everyday partner in the lab, Andreas Rost for putting up with my temperament and at times take charge of most of the lab with me. Thanks to Andrew Berridge for putting theory at my level of understanding. I am grateful to Reg Gavine, without whom cryogenics would not be possible. Thanks to Andreas, Andrew, Jason, Naoki, Alexandra, Jan, Demian, Patrick and Anne-Christine for making life in the lab so much fun.

I wish to thank Dr. Michael Sutherland for providing me the opportunity to work in the Cavendish Laboratory, guiding me through my experiments with the Big Fridge. I am grateful to him for allowing me to spend so much time in Cambridge. I thank particularly Swee Goh and Eoin O'Farrell for all the time that they spent with me on my experiments. I thank Mike, Swee, Eoin and Dr. Sibel Özcan for making my stay there very enjoyable. 

Finally, I would like to thank my partner in life Dr. Véronique Pagé, for all the encouragement and for supporting me in everything I do. This new life in Scotland and England would not have been the same without her at my side. I also thank our friends that were here or still are, James, Joachim, Elisabeth, Dimali and Paul.

The Overseas Research Students Awards Scheme (ORS), le Fonds Québécois de la Recherche sur la Nature et les Technologies (FQRNT), the Engineering and Physical Sciences Research Council (EPSRC) the University of St Andrews have funded my research and stay in St Andrews.


 

==> TeXShop_3839_201005291_16/Chapter3.tex <==

\chapter{Experimental methods and analysis procedures}
%---------------------------------------------------------------------------

This chapter aims at describing in details all the experimental techniques and the numerical methods that were used during this research project. These can be divided into two categories, namely those that relate to the de Haas van Alphen experiment, and those that are part of the procedure that was used for sample characterisation and sorting for single crystals of \TTS. 

The dHvA experiment is a standard one, but some of its details are often overlooked in the litterature. Thus, the author of this thesis found it relevant to bring it to the reader with its most intimate details. In particular, some aspects of the data analysis are quite obscure in the standard textbooks. Moreover, special steps can be taken in the numerical methods to tackle our specific aims, in particular for the dependence of the thermodynamic cyclotron mass on the magnetic field. 

The most important part of this chapter is the description of the main experiment, the measurement of the de Haas van Alphen effect, but as it will be shown, it cannot be carried out on any random sample. The purity requirements are extremely high, and they were not even yet achieved by the crystal growers in the early stages of this research project. Instead, the highest purity was reached by Robin S. Perry in a collaboration we have made over several months, where he was using the information that was provided by the characterisation and sorting procedure of section \ref{sect:search}. Moreover, even when a crystal grower is able to obtain very high purity levels, he still cannot predict with certainty the purity level of a grown single-crystalline rod. It generally varies spatially, so every rod has to be cut in several pieces, each of which have to be analysed independently. Consequently, this part of the project has been critical for the subsequent measurements of dHvA oscillations and will be described extensively.

This chapter will first present the dHvA experiment using the field modulation method, AC susceptibility. Next will be given the complete description of the various data analysis procedures. It will be followed by  a section relating to the rigourous checks that were made to ensure proper thermal equilibrium of the system. The second category of techniques will be introduced at this point, with first the AC susceptibility probe that we have built to be used with the adiabatic demagnetisation refrigerator. The complete procedure for characterisation and sorting of samples will follow with the other already established techniques, along with data relating to the purest samples.

\newpage
\section{AC susceptibility in a $^3$He/$^4$He dilution refrigerator}
\subsection{Basics of AC susceptibility with equations}

Magnetic measurements using AC susceptibility are very simple. The principle is to induce oscillations in the magnetisation of a sample and to measure the change in the magnetic field surrounding it using a coil. In order to improve sensitivity, we usually connect another empty identical coil to the first in opposition, in order to make this measurement a differential one. When measuring susceptibility as function of magnetic field, as it will be our case, we use a small oscillating magnetic $H_{AC}$ field on top of a very large slowly varying field $H_{DC}$:
\bea
H(t) &=& H_{DC}(t) + H_{AC}(t),\nn\\
&=& \alpha t + H_{AC}sin(\omega t).
\eea
The magnetic induction in the first coil is
\beq
{B(t)\over \mu_0} = H(t) + M(t),
\eeq
and the voltage on its terminals is
\beq
V_1 = {d\Phi \over dt} = A {dB\over dt} = A\mu_0 ({dH\over dt} + {dM\over dt}).
\eeq
The voltage on the second coil being
\beq
V_2 = A \mu_0 {dH\over dt},
\eeq
the substraction will leave, for the differential voltage
\beq
\Delta V = A \mu_0 {dM\over dt},
\label{eq:deltaV}
\eeq
and since the magnetic susceptibility $\chi$ is defined as
\beq
\chi = \chi' + i\chi'' = {dM\over dH},
\eeq
then
\beq
\Delta V = A \mu_0 \dot{H} \chi.
\label{eq:deltaVchi}
\eeq
The magnetisation, as a function of magnetic field, is usually a non-linear function, such that if we set our phase sensitive device for detection at higher harmonics, we should still obtain a signal. Let us expand the magnetisation as function of the small oscillating field:
\beq
M(H) = M(H_{DC}) + {dM \over dH}\bigg|_{H_{DC}} H_{AC} + {d^2M \over dH^2}\bigg|_{H_{DC}} {H_{AC}^2 \over 2} +  {d^3M \over dH^3}\bigg|_{H_{DC}} {H_{AC}^3 \over 6} + ...
\eeq
We want its derivative as function of time. We will assume the DC component to be independent of time:
\bea
{dM \over dt} &=& {dM \over dH}\bigg|_{H_{DC}} \dot{H}_{AC} + {d^2M \over dH^2}\bigg|_{H_{DC}} H_{AC}\dot{H}_{AC} + {d^3M \over dH^3}\bigg|_{H_{DC}} {H_{AC}^2\over 2}\dot{H}_{AC} + ... \nn\\
&=& {dM \over dH}\bigg|_{H_{DC}} H_{AC} \omega \cos(\omega t) + {d^2M \over dH^2}\bigg|_{H_{DC}} {H_{AC}^2\over 2} \omega \sin(2\omega t) \nn\\
&&+ {d^3M \over dH^3}\bigg|_{H_{DC}} {H_{AC}^3 \over 8}\omega(\cos(3\omega t) + \cos(\omega t)) + ...
\label{eq:Mexpansion}
\eea
Two things are to be observed from this equation: first, that the $n$th term corresponds to the $n$th harmonic, that is, if we keep only the lowest power of $H_{AC}$ for each harmonic, and is multiplied by the oscillating field to the power $n$. Second, the phase changes by 90$^{\circ}$ at each harmonic. 

Let us note here that there was an approximation that was taken for the derivative of the magnetisation: each derivative with respect to field is time dependent through the slowly varying field $H_{DC}$, but we have assumed that all the time dependence was within the oscillating field. In general, this has very little significance. It has an important effect when the magnetisation oscillates as function of magnetic field, during dHvA experiments, but to take into full account the time dependence is complicated. The next section will give the result, with the complete calculation given in appendix \ref{App:B}.

\subsection{Oscillatory signal in the field modulation method \label{sect:oscsignal}}

During dHvA experiments, the magnetisation, like the resistivity, follows oscillations as function of the inverse magnetic field, of frequency $F$, that we will take as sinusoidal (each oscillation harmonic, not to be confounded with detection harmonic, can be treated independently):
\beq
M(H) = M_0(H) + A \sin\bigg({2\pi F \over \alpha t + H_{AC}\sin(\omega t)}\bigg),
\eeq
where $M_0$ represents the magnetic background that is not oscillatory as function of magnetic field.
This is a function that is quite awkward to use, and we want it in a form that involves harmonics for our phase sensitive device. We will use the fact that the oscillating field amplitude is much smaller than the size of the DC field (usually by factor of about 10$^4$), 
\beq
{1\over H_{DC}(t) + H_{AC}(t)} \simeq {1\over H_{DC}(t)} - {H_{AC}(t) \over H_{DC}^2(t)},
\eeq
so that 
\bea
M(H) &\simeq& M_0(H) + A \sin\bigg({2\pi F \over H_{DC}}\bigg)\cos\big(\lambda \sin(\omega t)\big)\nn\\
&&-  A\cos\bigg({2\pi F \over H_{DC}}\bigg)\sin\big(\lambda \sin(\omega t)\big),
\eea
with 
\beq
\lambda = {2\pi F H_{AC} \over H_{DC}^2}.
\eeq
We are still left with the complicated factors $\cos(\lambda \sin(\omega t))$ and $\sin(\lambda \sin(\omega t))$. These are periodic functions and they can be expanded in Fourier series:
\beq
\cos(\lambda \sin(\omega t)) = a_0 + \sum_{n=1}^{\infty} a_n \cos(n\omega t) + b_n \sin(n\omega t),
\eeq
and so on. This calculation is given in appendix \ref{App:B} and the result involves Bessel functions of the first kind $J_k(\lambda)$:
\bea
M(H) &=& M_0(H) + A \sin\bigg({2\pi F \over H_{DC}}\bigg)\bigg( J_0(\lambda) + 2 \sum_{k=1}^{\infty}J_{2k}(\lambda) \cos(2k \omega t)\bigg)\nn\\
&&-  A\cos\bigg({2\pi F \over H_{DC}}\bigg)\bigg( 2 \sum_{k=1}^{\infty}J_{2k-1}(\lambda) \sin\big((2k-1) \omega t) \bigg).
\eea
We see that each harmonic has as a prefactor the Bessel function of order $k$, and as we showed in the last section, the magnetisation oscillations will be in phase with $H_{AC}$ for the odd harmonics and ${\pi \over 2}$ out of phase for the even ones. 

To calculate the differential voltage, we want the time derivative. In real systems, usually $M_0$ has much slower variations than the oscillations, so that all the higher derivatives are negligible, except, for instance, very close to a phase transition. We will then neglect the higher derivatives of $M_0$:
\bea
{dM \over dt} &=& {dM_0 \over dH} \big(\alpha + H_{AC}\omega \cos(\omega t)\big) +  2\omega \sin \bigg({2\pi F \over H_{DC}}\bigg) \sum_{k=1}^{\infty} 2k J_{2k}(\lambda) \sin(2k\omega t)\nn\\
&&-  2\omega \cos \bigg({2\pi F \over H_{DC}}\bigg)  \sum_{k=1}^{\infty} (2k-1)J_{2k-1}(\lambda) \cos\big((2k-1)\omega t\big).
\label{eq:dMdt}
\eea


It is clear in this result that the slowly varying magnetic background will be only present in the first harmonic, so that it can, as in our case with \TTS, be useful to use second or higher harmonic detection.

It seems surprising to find that the dHvA signal should be proportional to a function that oscillates with the AC field value. Let us look at this more closely. If the peak to peak value of the AC field should come close to the DC field interval it takes, at a certain DC field value, to complete a cycle for a certain dHvA frequency, then this cycle should be smeared out. The condition for zero amplitude on this frequency would be:
\beq
2 H_{AC} = \Delta H_{DC},
\eeq
where, for a cycle,
\beq
{1 \over F} = {1\over H_2} - {1\over H_1} = {\Delta H_{DC} \over H_{DC}^2},
\eeq
so that the condition for zero amplitude is
\beq
{2 H_{AC} F \over H_{DC}^2} = 1 =  {\lambda \over \pi}.
\eeq
This is approximately true, since the bessel function $J_1(\lambda)$ has its first zero at $\lambda \simeq 3.81$. The reason for this is that the DC field continuously changes, so that it actually takes a value for the oscillating field to be just a little over half the DC field interval. 

\begin{figure}[t]
	\begin{minipage}[t]{7cm}
		\begin{center}
		\includegraphics[width=7cm]{\PchapterIII besselj.eps}
		\end{center}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{7cm}
		\begin{center}
		\includegraphics[width=7cm]{\PchapterIII besselh.eps}
		\end{center}
	\end{minipage}
	\caption{($Left$) Bessel functions of the first kind. The case of $n=1$ is approximately linear at low values of $\lambda$ and has a first zero close to $\lambda = \pi$. The $n=2$ case is quadratic for small values of $\lambda$. (Right) Bessel functions of the first kind $J_k(\lambda)$ as function of the DC magnetic field $H_{DC}$ for $k=1,2$, for a frequency $F = 1.8$ kT and an oscillating field value of $H_{AC} = 16 G$.}
	\label{fig:bessel}
\end{figure}

Finally, as we also show in appendix \ref{App:B}, when $\lambda < 1$, the time derivative of $M$ reduces to a simpler expression, since
\beq
J_k(\lambda) \simeq {\lambda^k \over 2^k k!}.
\eeq
which indicates that in that case, each harmonic $k$ has an amplitude proportional to $H_{AC}^k / H_{DC}^{2k}$, a fact that will be useful in our work. In section \ref{sect:dHvAanalysis}, we will analyse the dependence on $H_{DC}$ of the oscillation amplitude, and normally, the functions $J_k(\lambda)$ have one that is not simple, unless $\lambda < 1$. In that case, we can multiply our signal by $H_{DC}^{2k}$ and get rid of the field dependence of the Bessel function prefactor. In the system of interest, \TTS, the highest frequency is below 10 kT and the lowest field where we still detect oscillations is 3 T, so that
\beq
\lambda = {2 \pi (10^4 \textrm{T})H_{AC} \over (9 \textrm{T}^2)} < 1\Rightarrow H_{AC} < 1.4\times10^{-4}\textrm{T} = 1.4 \textrm{G}.
\eeq
In all magnetic fields above 3 T, this value is much larger, and at 7 T, near our region of interest, it is 8 G.

Figure \ref{fig:bessel} show the bessel functions of the first kind. On the left panel, we see $J_k(\lambda)$. We can easily see that for the first harmonic ($k=1$), at values of $\lambda$ below 1, for a constant noise level, the signal to noise ratio will be proportional to the oscillating field, while for the second harmonic it will be quadratic. It will be easier to observe the first harmonic than the second at values of $\lambda \lesssim 2.2$. However, if the background magnetic signal is very large and slowly varying, sensitivity is lost and this will most probably result in digitised data and higher noise. In that case, even if the second harmonic is an order of magnitude or two smaller in amplitude compared to the first, one will gain in signal to noise ratio by using detection at $2\omega$. The right panel of fig. \ref{fig:bessel} shows the behaviour of the $k=1,2$ bessel functions for fixed dHvA frequency and oscillating field, as function of DC field. One must always remember that $\lambda$ is function of the DC field, so that the system can end up at a zero of the bessel function at low values. It is important to set the oscillating field such that for all DC field values, the system doesn't cross a zero of the $n$th bessel function when using the $n$th harmonic.


\subsection{The $^3$He/$^4$He dilution refrigerator}

\subsection{The experimental apparatus for dHvA measurements in the $^3$He/$^4$He dilution refrigerator \label{sect:plasticprobe}}

The dHvA experiment requires slow magnetic field ramps between zero and the largest value possible for the DC field, which is 17 T in our case. However, the AC field can be very small, and should be as small as possible while still producing a detectable signal, and we use values the order of 1-10 G in our experiments. This is because the oscillating field can be a source of heat through eddy currents, the power dissipation of which is proportional to the rate of change of the magnetic field. For a conducting cylinder of cross-sectional area $A$ and resistivity $\rho$ in a changing field, the power dissipation is
\beq
P_{eddy} \propto A {\nu^2 \dot{B}^2 \over \rho}.
\label{eq:eddy}
\eeq
We can see from this that we can reduce eddy current heating by either reducing the size of the conductor, the rate of change of the field, or increasing its resistivity. 

The first measurements done in our group of dHvA oscillations  \cite{borzi} were carried out on an insert for the dilution refrigerator that was made out of copper and stainless steel. This was good for having the best thermal equilibrium in the sample region of the magnetic field, but of course, copper being a good electrical conductor, the probe heated itself with any AC field greater than 0.1 G. With the samples of purity of 0.3-0.7 $\mu\Omega$cm that were available, with such an AC field, there was no chance of observing the second harmonic, even with the very low noise levels of the system, that were of around 30 pV/$\sqrt{Hz}$. As a result, the possibilities were limited by the large metamagnetic background signal in the first harmonic and another design for a probe that could work with higher oscillating fields was desirable. 

A second very similar probe was built (by R. A. Borzi) out of Tufnol, a type of hard plastic that has low thermal contraction at low temperatures, and it is the one used throughout this work. Figure \ref{fig:plasticprobe} shows a photo of this apparatus (left), and a diagram of the coil pair (right). All the wiring and the heat sinking was made such that eddy currents could only be present in the samples themselves. It supports two pick-up coils are made of 25$\mu$m wire with a few thousands of turns, and have a bore size of 2 mm in diameter. It has, like the first probe, a mechanism that  rotates them, with the samples they contain, in the magnetic field. It is thus possible to measure the susceptibility as function of angle.

\begin{figure}[t]
	\begin{minipage}[t]{8cm}
		\begin{center}
		\caption{Schematics of a pair of coils used in the plastic probe for the dilution refrigerator.}		
		\end{center}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{6cm}
		\begin{center}
		\includegraphics[width=3cm]{\PchapterIII ACsusc.eps}
		\end{center}
	\end{minipage}
	\label{fig:plasticprobe}
\end{figure}

Since electrical connections are used for the transport of heat at low temperatures (see \cite{pobell}), the outer surface of the plastic cylinder supporting the rotation mechanism is covered with coil foil, that is connected with a copper braid, which itself is normally screwed tightly to the mixing chamber of the dilution refrigerator. It is designed for allowing the heat inside the plastic to escape during cooldown of the system. However, since this plastic is insulating, we still expect the system to cool very slowly compared to the copper probe. Moreover, plastics are amorphous, and amorphous materials relax extremely slowly, releasing heat throughout their lifetime until they become crystalline. It is difficult to determine exactly how long it takes for this apparatus to be cold enough, after cooldown of the refrigerator, so that the temperature of the samples can be trusted to be the same as the mixing chamber. We have determined that waiting 24 hours when running the refrigerator at base temperature was enough, by measuring two consecutive dHvA field sweeps that lasted 12 hours each, the first starting 12 hours after cooldown. At the end of the first sweep, the amplitude of the oscillations are identical to those in the second one.

The probe was carefully designed for adequate cooling of the samples with very good electrical connections. A pure silver wire, of thickness 0.1 mm, is used as a separate cooling system from the one for the plastic (see the green wire in fig \ref{fig:plasticprobe}. It was baked in vacuum for one day in order to anneal its defects. The samples are electrically connected to this wire, which is in turn tightly screwed to the mixing chamber. Three gold wires per sample, of thickness of 25 or 50 $\mu$m, are used to connect these to the silver wire, using silver paint. It is a standard method used by most low temperature physics research groups. Section \ref{sect:eddy} will describe how to insure that the samples are at the same temperature as the thermometer.


\newpage
\section{De Haas van Alphen data analysis : numerical approaches \label{sect:dHvAanalysis}}

\subsection{Analytical expression for the oscillations}

We will first, for this section, give a reminder of the analytical expressions for the different dependences of the quantum oscillations on the different physical parameters, that were derived in the first chapter. This will be done in a compact form that will make the description of the numerical methods easier. It is quite important to understand the behaviour of these various expressions to understand the different problems that will be encountered when carrying out an analysis of dHvA data. 

We will write the expression for the oscillations using three functions, that we will call $J_k$,$LK$, $D$ and $E$, relating to the Bessel function modulation (eq. \ref{eq:dMdt}, through \ref{eq:deltaV} and \ref{eq:deltaVchi}), the Lifshitz-Kosevitch factor (eq. \ref{eq:LK}), the Dingle factor (eq. \ref{eq:D}) and the finite size of a real data set. We will use the variables $X$, and $T$ for the inverse field and temperature, and the integers $n$ and $k$, to identify the various Fermi surface sheets and the various detection harmonics. Also, we will use $F$ as the reciprocal variable to $X$, the oscillatory frequency, and $X_0$ as the average inverse field. 
The complete expression for the oscillatory part of the susceptibility in a dHvA experiment is
\beq
\chi \propto \sum_{n,k = 1}^\infty J_k(X, F_n) E(X-X_0) LK_n(X,T,m^*_n) D_n(X,m^*_n) \cos(2 \pi F_n X).
\label{eq:Fullosc}
\eeq

Let us start analysing these terms with the Bessel function prefactor $J_k$. As seen in section \ref{sect:oscsignal}, the oscillations will be modulated by Bessel functions of the first kind
\beq
J_k(\lambda_n) = J_k\bigg({2\pi F_n H_{AC} \over H_{DC}^2}\bigg) = J_k(2\pi F_n H_{AC} X^2).
\eeq
This is a complex modulating function, except if $\lambda_n < 1$, in which case we have that (see appendix \ref{App:B})
\beq
J_k(\lambda) \simeq {\lambda^k \over 2^k k!}  \propto {X^{2k} \over 2^k k!}.
\eeq
In this case, it is easy to get rid of the field dependent modulation produced by the field modulation method for AC susceptibility measurements; one needs to divide the data by $X^{2k}$, where $k$ is the detection harmonic number. Consequently, we will no longer refer to the Bessel functions and assume that all measurements for which we are interested in the amplitude modulation will be carried out with the condition that $2\pi F_n H_{AC} X^2 < 1$, and the data multiplied by $H^{2k}$.

The most important bit of this expression is the Lifshitz-Kosevitch (LK) function $LK(X,T)$, that relates to the smearing of the quantum jumps in the density of states at the Fermi surface due to thermal broadening of the Fermi surface,
\beq
LK_n(X,T) = {C_n X T \over \sinh C_n X T},
\eeq
with the variable $C_n$ containing various parameters, in particular the quasiparticle masses $m^*_n$,
\beq
C_n = {2 \pi k_b m^*_n \over e \hbar } \simeq 14.7 m^*_n.
\eeq
This variable is usually considered a constant, as normally the quasiparticle mass is a constant relating to a specific Fermi surface sheet, but in our quantum critical case, it will not be, so that we should write
\beq
m^*_n = m^*_n(X).
\eeq 
Of course, the mass will vary in a much slower fashion compared to the oscillations themselves.

Figure \ref{fig: LKsurf} illustrates the dependence on $T$ and $X$ of the LK factor. It is of course the same for both variables, but the values that can be reached in an experiment are not the same. Very often, a small region in $X$ will be used, where the LK factor varies very little, and the value of $X$ can be safely replaced by its average, $X_0$. In a case where a large $X$ interval has to be used, the dependence on $X$ will have to be considered. The implications of this will be shown in the next two sections.

Finally, we note here that the LK factor contains the only dependence on $T$ in the full expression for the oscillations.

Next, we have the Dingle factor $D(X)$, that takes into account the scattering due to imperfections in the crystal lattice,
\beq
D(X) = e^{-\lambda_n |X|},
\eeq
with the constant $\lambda_n$ being
\beq
\lambda_n = {2 \pi k_b m^*_n T_D \over e \hbar } = C_n T_D \simeq 14.7 m^*_n T_D,
\eeq
and $T_D$ the Dingle temperature, which is proportional to the scattering rate $\Gamma$,
\beq
T_D = {\hbar \over k_b} \Gamma.
\eeq

Finally, we have the envelope function $E(X)$. The primary reason for including this is first because of the fact that the data is always finite, in other words that we don't measure from zero to infinite magnetic field. But also, in the standard method to perform a Fourier transform on a data set, one uses what is called windowing, which I will explain in the next section. 

Consequently, we will always consider our data to extend from zero to infinite $X$, to be symmetric around zero and to be zero for all $X$ except where $E(X)$ is not zero, which corresponds to our measurement interval. 

\begin{figure}[h!]
\begin{center}
	\includegraphics[width=.7\columnwidth]{\PchapterIII LKsurf.eps}
	\caption{Three dimensional representation of the Lifshitz-Kosevitch factor as function of temperature $T$ and inverse magnetic field $X$, for a constant mass $m^*$. The shaded region illustrates the possible measurement interval for these variables, where the magnetic field extends between 6 and 15 T. The white line indicates $X_0$, the average value for $X$ one would have if one used this whole interval. One can see that the dependence is the same for $X$ and $T$ but the measurement intervals for these variables is not. For smaller field intervals, the dependence on $X$ can very often be considered constant and $X$ can be replaced by $X_0$. }
	\label{fig: LKsurf}
\end{center}

\begin{center}
	\includegraphics[width=.65\columnwidth]{\PchapterIII D.eps}
	\caption{Illustration of the Dingle factor as function of $X$. It is symmetric around infinite magnetic field and zero at zero field ($X \rightarrow \infty$).}
	\label{fig: D}
\end{center}
\end{figure}


\subsection{Fourier transforms and windowing \label{sect:FFTwindowing}}

In order to study the Fermi surface structure of a material, we want to separate the different contributions at different frequencies from its various sheets. For that, we will of course use a Fourier transform. Unfortunately, it is not obvious what the analytical Fourier transform of equation \ref{eq:Fullosc} is. But, by using the convolution theorem, we can discover a few useful things. 

We expect the result of the Fourier transform to have the form of a power spectrum composed of peaks of a certain width, at specific frequencies $F_n$. The convolution theorem tells us that the transform of a product of functions is equal to their convolution in reciprocal space,
\bea
\mathcal{F}[f(x)g(x)] &=& \mathcal{F}[f(x)] \ast \mathcal{F}[g(x)],\nn\\
&=& \tilde{f}(x) \ast \tilde{g}(x).
\eea
Applied to our expression, we get
\beq
\mathcal{F}[\chi(X,T)] \propto \sum_n \tilde{E}(F) \ast \bigg(\tilde{D_n}(F) \ast \big( \tilde{LK}(F,T) \ast (\delta(F-F_n) + \delta(F+F_n))\big)\bigg),
\eeq
where, of course, the Fourier transform is taken as function of $X$ and yields functions of the frequency $F$.

Let us first suppose $D$ and $LK$ to be constants, in order to study $E$. In that case, the Fourier transform will be proportional to 
\beq
\sum_n \sum_\pm \tilde{E}(F \pm F_n),
\eeq
which is the Fourier transform of the envelope $E$ centred at $\pm F_n$. If the data of a dHvA set extends from zero to infinite magnetic field, $\tilde{E}(F \pm F_n)$ will be a Dirac delta function centred at $\pm F_n$. In a real physical case,  $\tilde{E}(F \pm F_n)$ will have a width and a shape. Let us take $E(X)$ to be a top hat function of width $2a$ centred at $X_0$, equal to one where dHvA data exists, and zero everywhere else. Then, $\tilde{E}(F \pm F_n)$ will be
\beq
\tilde{E}(F) = {1\over \sqrt{2\pi}}\int_{X_0 - a}^{X_0 + a} e^{-iFX}dX = {2\over \sqrt{2\pi}}e^{-iFX_0} {\sin(aF) \over F} = {2\over \sqrt{2\pi}}a e^{-iFX_0} \sinc(aF).
\eeq
When we take the modulus of this result, it oscillates around a central peak, so that its satellite peaks can be misinterpreted as different dHvA frequencies. It is then useful to use another form for $E(X)$, and in particular, that decreases smoothly to zero at the edges of the data set. This is called windowing. 

The only function of which the Fourier transform does not oscillate is a Gaussian. Unfortunately, it is also never zero, so that to be used here, it would have to be truncated to zero at the edges of the data set, and is not ideal. Instead, there are two widely used windowing functions similar to a Gaussian, that are based on a truncated cosine function, the Hann and the Hamming windows. The first is defined as
\bea
E(X) &=& .5 + .5 \cos \bigg[{\pi \over a} (X - X_0)\bigg], \quad -a < X-X_0 < a \nn\\
&=& 0 \quad otherwise.
\eea
Its Fourier transform is
\beq
\tilde{E}(F) = {1\over \sqrt{2\pi}}e^{iFX_0} \sinc(aF) {a \pi^2 \over \pi^2 - a^2F^2},
\eeq
and decreases much faster than the $\sinc$ function away from the main peak, having much smaller satellite peaks. The Hamming window, on the other hand, is tuned with a parameter $\alpha$ to suppress to zero the first satellite peak on each side of the main peak and is obtained by adding a very small top hat window with a Hann window:
\bea
E(X) &=& \alpha + (1-\alpha) \cos \bigg[{\pi \over a} (X - X_0)\bigg], \quad -a < X-X_0 < a \nn\\
&=& 0 \quad otherwise.
\eea
The value of $\alpha \simeq 0.54$ gives the best results. Its Fourier transform is
\beq
\tilde{E}(F) = {2a \over \sqrt{2\pi}}e^{iFX_0} \sinc(aF) \bigg(\alpha + (1-\alpha){a^2F^2 \over \pi^2 - a^2F^2}\bigg),
\eeq
The windowing procedure will be very important in order to obtain dHvA spectra of which we can easily distinguish the various frequencies present. 

Finally, one useful comment to add is about the width of these functions. The half width at half maximum of the $\sinc$ function is found by equating
\bea
{2a\over \sqrt{2\pi}} {\sin(a \Delta F) \over a \Delta F} &=& {a \over 2} \nn\\
\Rightarrow \sin(a \Delta F) &=& {a \Delta F \over 2},
\eea
which yields numerically $a \Delta F = 0.3017$, where $\Delta F$ is measured from the centre of the function. The same can be done with the Hann and the Hamming windows, which give, respectively, 
\bea
\Delta F = 0.3017/a &&\quad Top\quad Hat \nn\\
\Delta F = 0.5 / a &&\quad Hann\nn\\
\Delta F = 0.4538 / a &&\quad Hamming
\eea
It means that a Fourier transform taken on a set of data of any possible frequency (premitted by the sampling rate) will produce a peak in the spectrum of which the width will be determined only by that of the window, or the size of the data set, $regardless$ of, for instance, the number of cycles of oscillation within that set. For one to be able to compare spectral data of different frequencies from different data sets, the Fourier transforms have to be performed with equal inverse field widths, not the same number of cycles of oscillation.

\subsection{Units with Fourier transforms}

As we saw with the analytical expressions for the oscillations, the functions $LK(X,T)$ and $D(X)$ vary in a much slower fashion than the oscillations themselves. This generally allows us to take them as constant and out of the Fourier transform:
\beq
\tilde{\chi}(F,T) \propto \sum_{n,\pm} LK_n(X_0,T) D_n(X_0) e^{iFX_0} \tilde{E}(F \pm F_n)
\label{eq:fullFT}
\eeq
It is written here as the Fourier transform of the magnetic susceptibility. We actually measure, in a differential susceptibility measurement, a voltage $\Delta V$ and don't necessarily know the proportionality factor between $\Delta V$ and $\chi$. Knowing with precision this number involves a complicated procedure and is not necessary for dHvA. But it can be important, as in our case, to be able to compare various dHvA signals measured on different samples of a same material. We then want Fourier transforms to be comparable to one another, and consequently, to have rigourous units.  As we measure voltages and take Fourier transforms as function of inverse field $X$ in T$^{-1}$, the frequency units are T and we expect that the units of the Fourier transforms should be $\textrm{V}/\sqrt{\textrm{T}}$. 

The Fourier transform is generally a complex number data set. The power spectrum $W(F)$, that, in signal processing theory, represents the power radiated per unit frequency, is the square of the modulus divided by the interval (that we denote $2a$):
\bea
W(F) &=&  {1\over 2a} \bigg| \int_{X_0-a}^{X_0+a} \Delta V(X) e^{-iFX}dX \bigg|^2,\nn\\
&=&{1\over 2a} \tilde{\Delta V}^*\tilde{\Delta V},
\eea
which has units of V$^2/$T. In this work, when we plot spectra, we plot the square root of the power spectrum, in $\textrm{V}/\sqrt{\textrm{T}}$. In order to know the voltage amplitude of the signal for a certain frequency interval, the power spectrum has to be integrated within that interval, which yields units of V$^2$, and then take a square root of the result. Due to spectral leakage, or in other words, the fact that the peaks in the power spectrum have a width and shape, in order to know the voltage amplitude of a certain dHvA frequency, we need in theory to integrate the power spectrum from minus infinity to infinity, since $\tilde{E}(F)$ is non-zero at all $F$. In practice, of course, the presence of multiple frequencies makes this impossible and one can integrate, for instance, only the central peak of $\tilde{E}(F)$ and multiply by two, since each dHvA frequency is present at $\pm F_n$. This should yield a fraction of the real amplitude, that depends only on the integration limits and the windowing function used in the Fourier transform. 

If 
\beq
\Delta V(X) = \sum_n A_n \cos(F_n X) 
\eeq
is the dHvA signal, with amplitudes $A_n$, in units of V, the Fourier transform we perform will be
\bea
\tilde{\Delta V}(F) &=& {1\over \sqrt{2\pi}} \int_{-\infty}^{\infty} E(X) \Delta V(X) e^{iFX} dX,\nn\\
&=& \sum_{n,\pm} A_n \tilde{E}(F\pm F_n),
\eea
so that
\beq 
W(F) = {1\over 2a} \bigg| \sum_{n,\pm} A_n \tilde{E}(F\pm F_n) \bigg|^2
\eeq
What we want to know are the amplitudes $A_n$. Let us assume that the frequencies are well enough separated so that the various $\tilde{E}(F-F_n)$ don't overlap. We then need to know the value of the integral of $|\tilde{E}(F)|^2$. In the case of a top hat windowing function, the integral is
\beq
\int_{-\infty}^{\infty} |\tilde{E}(F)|^2 dF =  \int_{-\infty}^{\infty} {4a^2 \over 2 \pi} \sinc^2(aF) dF = 2a,
\eeq
so that the total power of the $n$th frequency will be
\bea
W_n &=& A_n^2,\nn\\
\Rightarrow A_n &=& \sqrt{W_n} =  \sqrt{ \int_{-\infty}^{\infty} {1\over 2a}|\tilde{\Delta V}(F)|^2 dF}.
\eea
In the case of a Hann window, the integral is very tedious and gives
\beq
\int_{-\infty}^{\infty} |\tilde{E}(F)|^2 dF =  \int_{-\infty}^{\infty} {a^2 \pi^3\over 2} {\sinc(aF) \over \pi^2 - a^2F^2} dF = {3a \over 4},
\eeq
so that
\beq
A_n =  \sqrt{ {8 \over 3}\int_{-\infty}^{\infty} {1\over 2a}|\tilde{\Delta V}(F)|^2 dF}.
\eeq
Finally, with a Hamming window, the integral is
\beq
\int_{-\infty}^{\infty} |\tilde{E}(F)|^2 dF = 2a (\alpha^2 + {1 \over 2}(1-\alpha)^2),
\eeq
and with the usual parameter $\alpha = 0.54$, the result is ${1987 \over 2500}a = 0.7948a$.

Later in this thesis, when we quote signal levels, they are always obtained using this method, with a Hamming windowing scheme. The voltages thus calculated are directly comparable with noise levels, measured in $\textrm{V}/\sqrt{\textrm{Hz}}$, if we divide them by the square root of the lock-in amplifier time constant (which is 1 in most our experiments).

\subsection{Mass analysis \label{sect:mass}}

As we stated in the first chapter, one of the parameters of primary interest in dHvA studies is the cyclotron thermodynamic quasiparticle mass. This mass is extracted from the dHvA data from the temperature dependence of the amplitude of the oscillations, and one such mass can be obtained from each frequency in the dHvA spectrum, and consequently can be assigned to a specific branch of the Fermi surface. We will, in this section, explain the numerical method used to extract the quasiparticle masses.

Let us rewrite eq \ref{eq:Fullosc}:
\beq
\chi \propto \sum_n E(X-X_0) LK_n(X,T,m^*_n) D_n(X,m^*_n) \cos(2 \pi F_n X).
\eeq
We will once again assume that the functions $LK(X,T)$ and $D(X)$ vary slowly enough that we can take them out of the integral, by replacing $X$ by $X_0$. This is easily true most of the time and we will quantify in the next section the situations where it is $not$ possible to make this approximation, in other words, when the inverse field window is too large. Let us rewrite the Fourier transform of eq. \ref{eq:Fullosc}, that is, eq \ref{eq:fullFT}:
\beq
\tilde{\chi}(F,T) \propto \sum_{n,\pm} LK_n(X_0,T) D_n(X_0) e^{iFX_0} \tilde{E}(F \pm F_n)
\eeq
We see that the temperature dependence is solely in the function $LK_n(X_0,T)$,
\beq
LK_n(X,T) = {C_n X T \over \sinh C_n X T}, \quad C_n \simeq 14.7 m^*_n.
\eeq
In order to extract $m^*_n$, we need to perform a non-linear fit of the $LK$ function. This fit will be carried out on values of integrals calculated on peaks in the spectrum, as described in the last section, as function of temperature. The fit will normally have two adjustable parameters, $A$ and $m$:
\beq
LK_{fit}(X_0,T) = A {14.7 m X_0 T \over \sinh 14.7 m X_0 T}.
\label{eq:LKfit}
\eeq
It is possible, though, that the dHvA spectra have a constant additive offset, so it is also possible to use a three parameter non-linear fit,
\beq
LK_{fit}(X_0,T) = A {14.7 m X_0 T \over \sinh 14.7 m X_0 T} + C.
\eeq
This should be used with care, though, because background noise in spectra tend to increase with temperature, which would lead one to think of the presence of an offset constant to all temperatures, and could lead to small errors on the mass.

\subsection{Fourier transforms using large field windows}

$A$ $priori$, one doesn't know whether the field window used in a mass analysis is too large such that the functions $LK$ and $D$ vary enough to generate a significant error. In this section, we will show how to know whether the approximation to take them as constant is problematic, and that the error is always in the same direction, to say, that the approximation error $underestimates$ the mass. This problem is usually overlooked, as people generally use the standard recipe of dHvA analysis  presented in the previous section, but it has proven critical for one material studied in our group, Sr$_2$RhO$_4$ (???, ???), where the sum of the masses measured with the standard recipe did not initially agree with specific heat data taken on this material. The analysis presented in this section contributed in the finding of the "missing mass", the fact that the normal analysis underestimated the values of the masses, and the method to obtain the more accurate values that were published.

When one deals with a normal set of data, with well separated frequency peaks in the dHvA spectrum, one is not very limited in possible sizes of the inverse field window in which to perform a Fourier transform. Basically, noise will be the main limiting factor, as using a data set featuring more cycles of a frequency increases the peak height in the Fourier spectrum with respect to the noise. In a fairly clean set of data, as few as 10 cycles can be used and still well resolve the temperature dependence, as long as one is sure that the various dHvA peaks are separated well enough and do not mix. The only situation where one will need to use large field windows are if dHvA peaks are too close to one another or if the frequencies are too low.

Let us look at the amplitude of a peak in a dHvA spectrum. The initial Fourier transform is
\bea
\tilde{\chi}(F) &\propto& \sum_n \int_{-\infty}^{\infty} E(X-X_0) LK_n(X,T) D_n(X) \cos(2 \pi F_nX) e^{-iFX}dX,\nn\\
&=& \sum_{n,\pm} \int_{-\infty}^{\infty} E(X-X_0) LK_n(X,T) D_n(X) e^{\mp iF_nX}dX.
\eea
We take one of the dHvA frequencies near $F'$ and remove the subscripts $n$, so that
\beq
\tilde{\chi}(F') \propto \int_{-\infty}^{\infty} E(X-X_0) LK(X,T) D(X) e^{-iF'X}dX.
\eeq
Now the variable $F'$ is a frequency centred on a peak at $F_n$. Let us take the power spectrum and integrate it over a very small frequency interval $f$ from the centre of the peak,
\bea
W(f) &=& {1\over 2a} \int_0^f \bigg| \int_{-\infty}^{\infty} E(X-X_0) LK(X,T) D(X) e^{-iF'X}dX\bigg|^2dF',\nn\\
&\simeq& {1\over 2a} \int_0^f \bigg| \int_{X_0-a}^{X_0+a} E(X-X_0) LK(X,T) D(X)dX\bigg|^2dF',\nn\\
&=& {f\over 2a} |\big<E(X-X_0) LK(X,T) D(X)\big>|^2,
\eea
where the brackets mean the average of the product of the three functions. The smallest interval $f$, for a discrete Fourier transform, will correspond to the largest inverse field interval that we have, namely $2a$. Consequently, the value of the square root of the integrated power spectrum will be the average of the product of the functions,
\beq
\sqrt{W} = \big<E(X-X_0) LK(X,T) D(X)\big>.
\eeq
Let us assume for an instant that $D(X)$ is constant and that $E(X-X_0)$ is a top-hat window. Taking the square root, we see that the $T$ dependence we are looking for will be proportional to $\big<LK(X,T)\big>$.

We know that the width in temperature of $LK(X,T)$ varies with inverse field $X$. Consequently, averaging this function should give a $LK$-like function that cannot be adjusted adequately by a non-linear fit. But also, this average will be wider in $T$ than $LK(X_0,T)$, the $LK$ function $at$ the average field $X_0$, which is what we would adjust by a non-linear fit in the normal procedure. We would then obtain a mass that is smaller than the real value.

\begin{figure}[t]
\begin{center}
	\includegraphics[width=.6\columnwidth]{\PchapterIII Mass_B.eps}
	\caption{Relative value of the quasiparticle mass extracted with the normal fit of the LK relation (eq. \ref{eq:LKfit} applied on simulated dHvA data, with the size of the inverse field window varying, to the real imposed value. The relative mass is plotted as function of the position in $B = 1/X$ of the lower boundary of the window, the higher boundary fixed at 15 T, where the oscillations are the highest (imitating a real experiment). The frequency used was of 1 kT and the mass of 3 electron masses. We see that for a vanishingly small window, the calculation error is nil, and increases with the size of the window. The error can be higher than 50\%. }
	\label{fig:Mass_B}
	\end{center}
\end{figure}

Now, assuming that $D$ and $E$ are not constant, we see that the matter is even more complicated. These functions will make the average of the $LK$ function weighed differently at different values of $X$, $E$ towards the centre of the window and $D$ towards the higher values. But still, we know that the mass extracted by a fit of $LK(X_0,T)$ will underestimate the value.

Figure \ref{fig:Mass_B} shows $LK$ fits taken on simulated dHvA data, using the normal method of eq. \ref{eq:LKfit}, as function of the position of the lower boundary of the inverse field window, the higher one being fixed. We see that as the lower boundary moves towards the higher boundary (the window shrinks), the mass approaches the real imposed value.

This reasoning tells us two things. The first is that the function to fit, in a generally correct way, is
\beq
\big<E(X-X_0) LK(X,T) D(X)\big>.
\eeq
But this requires knowledge of the Dingle temperature $T_D$ for the function $D(X)$, so we will show how this parameter can be obtained in section ???. Second, the mass can also be found out in an auto consistent way using a simulation, and find the error on the fit.

Finally, we need a way to quantify the conditions for the applicability of the approximation of taking $D$ and $LK$ as constants. If one has well enough separated frequencies, one can find out if a calculated mass is accurate by reducing the size of the analysis window and checking for variations of the value. But in the case where dHvA peaks are too close to one another such that when reducing the size of the analysis window, the peaks are not well resolved from one another, then this is where the situation is more conplicated. 
In such a case, one has to calculate the Dingle temperature, using the method described further. One should also calculate, as a starting point, the "mass" of the integral of the whole unresolved peak structure, using the method of eq. \ref{eq:LKfit}, which should be some kind of average of all the masses of the frequencies involved. The half width at half maximum of the LK function in inverse field is
\beq
\Delta X_{LK} = {0.148 \over m^* T}.
\eeq
The same for the D function is
\beq
\Delta X_D = {0.05 \over m^* T_D}.
\eeq
The criterium should be that for values of $T$ where the LK function has an appreciable value at the values of $X$ within the inverse field window, these parameters should be very much larger than $2a$, the width of the window.
Of course, another criterium is the eye. In the problematic cases, one can see that the amplitude of the oscillations change by an order of magnitude or more across the inverse field window.

\subsection{The envelope extraction method \label{sect:envelope}}

Another method of relevance is described in the review on Sr$_2$RuO$_4$ by C. Bergemann $et$ $al.$ \cite{bergemann}, that is, the envelope extraction. By envelope, we mean here the low frequency modulation of the oscillations, which is of course again due to the product of the functions $D$ and $LK$. Using this method, which consists of filtering, one can obtain continuous functions of the modulation amplitude for all individual dHvA frequencies. I will briefly describe the method used for the extraction of the envelopes.

Let us assume oscillations of the form
\beq
G(X) = \sum_n A_n(X)\cos(F_nX),
\eeq
The functions $A_n(X)$ are the envelope we are looking for. Carrying out a Fourier transform yields
\bea
\tilde{G}(F)  &\simeq& \sum_n \int_{-\infty}^\infty A_n(X) \bigg({e^{iF_nX} - e^{-iF_nX} \over 2i}\bigg) e^{-iFX} dX,\nn\\
&\simeq& \sum_n{1 \over 2i}\int_{-\infty}^\infty A_n(X) (e^{i(F_n-FX} - e^{-i(F_n+FX}) dX,\nn\\
&\simeq& {1 \over 2i}\sum_n[\tilde{A}_n(F - F_n) - \tilde{A}_n(F + F_n)]
\eea
We now want to isolate one of the various $\tilde{A}_n(F)$, namely $\tilde{A}_m(F)$, by filtering the spectrum by using a window that leaves only one peak and sets the rest to zero. If we also set the negative frequencies to zero, (which are a reflection of the positive ones), we obtain,
\beq
\tilde{G}_{flt}(F) = {1 \over 2i}\tilde{A}_m(F - F_n).
\eeq
By an inverse Fourier transform, we should obtain the desired $A_m(X)$:
\bea
G_{flt}(X) &=& {1 \over 2i}\int_{-\infty}^\infty \tilde{A}_m(F - F_n) e^{iFX}dF,\nn\\
&=& {1 \over 2i}\int_{-\infty}^\infty \tilde{A}_m(F') e^{i(F' + F_n)X}dF',\nn\\
&=& {1 \over 2i} \tilde{A}_m(X) e^{i(F_n)X}.
\eea
If we take the modulus, we are left with the envelope, without oscillations:
\beq
|G_{flt}(X)| = {1 \over 2} |A_m(X)|.
\eeq

It should be possible to use this method even if the frequency peaks are close to one another. The factor that can make it difficult is if the dHvA frequencies vary with inverse field, as it is the case with \TTS close to the metamagnetic transition. If it is not the case, a very narrow filter window can be used. The shape of the filter window is very important for exactly the same considerations as for the function $E$. The resulting envelope extracted by this method will consist of the real envelope convolved with the Fourier transform of the filter function. For instance, using a top hat filter will lead to oscillations in the extracted envelopes. If the frequencies change with $X$ but are well separated, one can use a top hat window that is wide enough to include all necessary information in the spectrum related to one frequency, but with its corners "rounded":
\beq
\sqrt{2} \sigma \bigg[ \erf({F-a \over \sqrt{2}  \sigma}) - \erf({F+a \over \sqrt{2}  \sigma})\bigg],
\eeq
where $\sigma$ is the "roundness" of the filter and $\erf$ is the error function. The rounder the filter, the more it will look like a gaussian and the less oscillations will be present in the result.

The usefulness of this method is multiple. One of the reasons for our interest is that it makes possible the fit, using eq. \ref{eq:LKfit}, of the LK relation at each value of the inverse field $X$. This makes the calculated quasiparticle mass absolute for a value of $X$, instead of an average over the window $E$ used in a Fourier transform. If the mass is a constant, this is of very limited interest, but when it is not, as in the case of \TTS, one can calculate the field dependence of the mass with this. We must note here though that the LK fits, when using this method, are quite noisy.

The other interest in this method is in the envelopes themselves at the lowest temperature. As I will show in the next section, it is possible to extract the Dingle temperature with this method.

\subsection{The Dingle analysis}

Let us rewrite once more eq \ref{eq:Fullosc}:
\beq
\chi \propto \sum_n E(X-X_0) LK_n(X,T,m^*_n) D_n(X,m^*_n) \cos(2 \pi F_n X).
\eeq
We know that when the temperature is strictly zero, the LK function is a constant of the inverse field. In a real physical experiment, it is always possible to find a temperature for which there will be a region of inverse field where $LK(X,T)$ will be always very near to equal to one. In such a case, the amplitude function will depend only on $D(X)$. In one can extract by one way or another the amplitude as function of $X$, then a fit of this as function of $X$ with the appropriate exponential,
\beq
D(X) = e^{-\lambda |X|}, \quad \lambda = 14.7 m^*T_D,
\eeq
and extract the Dingle temperature $T_D$.

This can be achieved by the envelope extraction method presented in the previous section, or equivalently by convolving the data with a cosine function (if the frequencies are constants of $X$). This can also be achieved by using the $A$ parameter of the fit of eq \ref{eq:LKfit}, if one uses small enough inverse field windows. For instance, one can use as few as 10 cycles of oscillation of the frequency of interest in the inverse field window, or as few as needed to resolve the frequency peak in the spectrum above the noise. One must perform Fourier transforms over such a small window and move it along inverse field. If one allows the windows to overlap, one can in principle obtain one value of $A$ per cycle of oscillation.


\newpage
%------------------------------------------------------------------------------------------------

\section{Preliminary experiments: reproducing previous work \label{sect:preliminary}}

During the early days of this thesis project, it has been possible to perform dHvA experiments in order to test the new apparatus design described in section \ref{sect:plasticprobe}, which allows the use of large excitation fields and second harmonic detection, and obtain some preliminary results. The aim there was to reproduce the work that was done already by R. A. Borzi $et$ $al.$\cite{borzi} in the same laboratory in St-Andrews, but with second harmonic detection. We will present here this preliminary work, in order to introduce the reader to the dHvA data of \TTS, but also as a standard for comparison of the quality of data in later stages of this research. In section \ref{sect:search}, in particular, we will study the quality of various crystals of \TTS, and this data will allow us to predict which ones will produce better quality measurements.

This section is divided into two parts. In the first, we present the dHvA data and Fourier transforms away from the QCEP. In the second, we will study the evolution of various quantities near the QCEP.

\subsection{dHvA oscillations and spectra}

\begin{table}[htb]
	\begin{center}
		\begin{tabular}[h]{r|c c c c c|c c c}
			\hline
			&&&&&&&&\\
			&\multicolumn{5}{l}{Sr$_3$Ru$_2$O$_7$} & \multicolumn{3}{|l}{Sr$_2$RuO$_4$}\\
			&&&&&&&&\\
			\hline
			&&&&&&&&\\
			$F (kT)$ & $0.2$ & $0.5$ & $0.8$ & $1.8$ & $4.2$ & $3.0$ & $12.77$ & $18.66$\\
			$m^*/m$ & $6\pm3$ & $13\pm4$ & $10\pm1$ & $8\pm1$ & $9\pm2$ & $3.3$ & $7.0$ & $16.0$\\
			&&&&&&&&\\
			\hline
		\end{tabular}
		\label{tab:freqRAB}
		\caption{Table of reported values for frequencies and their corresponding quasiparticle masses for Sr$_3$Ru$_2$O$_7$ \cite{borzi} and Sr$_2$RuO$_4$ \cite{bergemann}.}
	\end{center}
\end{table}

In this first section, we will begin by showing the presence of the dHvA oscillations with a new sample of Sr$_3$Ru$_2$O$_7$. This sample was grown by R. S. Perry, who had also produced those used in the previous work done by Borzi $et$ $al.$. As we will show, it contains Sr$_3$Ru$_2$O$_7$ of average quality, but unfortunately also intergrowths of mainly Sr$_2$RuO$_4$. Both first and second harmonics were recorded at the same time during each experiment, using different lock-in amplifiers, in order to be able to compare data with the previous work, which was performed using a very low excitation field of 0.1 G and first harmonic. A modulating field of 16.5 G was used at a frequency of 41 Hz. We used a spectrum analyser to determine a frequency with low noise at its fundamental and second harmonic. Field sweeps were performed at a rate of 0.02 T/min, so that each of them, extending from 3 to 14.5 T, took around 12 hours to complete, and those measured at night feature the less noise. They were performed at various temperatures between 30 and 400 mK. The temperature was measured with a RuO thermometer, and the base temperature of the sample probe was obtained after waiting for 6 hours at full cooling power, as could be inferred from a negligible change in amplitude of the oscillations at the same field more than 12 hours later (after less time, for example 3 hours, the measuring apparatus was still not at the lowest temperature). All other sweeps at higher temperatures were measured in increasing order of temperature. 

The first important task was to reproduce previous results with second harmonic detection. The previous work reported peaks at frequencies shown in table \ref{tab:freqRAB}. Here, the same frequencies were detected, with roughly the same quasiparticle masses. But more frequencies were observed, and some of those were identified with two of the three seen in  Sr$_2$RuO$_4$ (table \ref{tab:freqRAB}). We also observed that this spectrum changes as one passes through the quantum critical region, near 7.8 T. We will enumerate the different dHvA frequencies observed below and above the metamagnetic transition field and identify them. But first, let's have a look at the oscillations themselves.
 
\begin{figure}[t]
  \begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII BothHarmOsc.eps}
	\caption{Oscillations for the first and second harmonics. The oscillations for $n=1$ are superimposed on the peaks in the real susceptibility $\chi_1 '$, while for $n=2$ they are superimposed on the imaginary $\chi_2 ''$, featuring sharp structures only very near the metamagnetic transitions around 7.8 T.}
	\label{fig:1nHarmOsc}
	\end{center}
\end{figure}

Figure \ref{fig:1nHarmOsc} shows oscillations for the first and second harmonics. The data for $n=1$ is essentially the same as what was observed previously, consisting in oscillations superimposed with the very wide susceptibility peaks of the metamagnetic transition. For $n=2$, except for a constant offset, the only non-oscillatory features appear at, in order as field increases, a cross-over and both metamagnetic transitions, between 7.5 and 8.5 T, the last two of which delimitate the recently reported quantum phase \cite{science2}. A closer look at the data reveals that the signal to noise ratio is extremely good, at least for the main frequency in the signal and that it is possible to follow the oscillations much closer to the transitions than for $n=1$.
 
 

\begin{figure}[h!]
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII BothHarmSpectra.eps}
	\caption{Frequency spectra for the first and second harmonics, with the Fourier transforms taken between 5.5 and 6.5 T.}
	\label{fig: BothHarmSpectra}
	\end{center}
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII BothHarmSpectra2.eps}
	\caption{Frequency spectra for the first and second harmonics, with the Fourier transforms taken between 9 and 12 T.}
	\label{fig: BothHarmSpectra2}
	\end{center}
\end{figure}

The main frequencies in the ranges where Fermi liquid is expected, away from the transitions on both sides, can be obtained by taking a simple FFT of the data over relatively large ranges of inverse field. Figures \ref{fig: BothHarmSpectra} and \ref{fig: BothHarmSpectra2} show such spectra for both harmonics, with the FFT calculated between 5.5 and 6.5 T in the low field region, and between 9 and 12 T for the high field region. No structure was seen beyond 12 kT in any of the spectra. The same peaks are seen in both harmonics, although the higher frequencies are better resolved with the second harmonic.  

\begin{table}[t]
	\begin{center}
		\begin{tabular}[h]{|c|c|c|c|}
			\hline
			\multicolumn{2}{|c|}{5.3 to 7.25 T} & \multicolumn{2}{|c|}{9 to 12 T}\\
			\hline
			Peak (kT) & $m^*/m$ & Peak (kT) & $m^*/m$\\
			\hline
			0.15 & $5.4 \pm 0.3$ & 0.13 & $6 \pm 1$\\
			0.45 & $11 \pm 2$ & &\\
			0.9 & $9 \pm 1$ & 1.1 & $10.4 \pm 0.4$\\
			& & 1.4 & $9 \pm 2$\\
			1.8 & $6.5 \pm 0.2$ & 1.6 & $6.3 \pm 0.2$\\
			2.8 & $4.6\pm0.2$ & &\\
			3.0 & $3.2\pm0.1$ & 3.0 & $3.0\pm0.3$\\
			& & 3.3 & $12\pm1$\\
			4.2 & $12\pm2$ & 3.9 & $12.5\pm0.3$\\
			& & 4.0 & $13.0\pm0.1$\\
			& & 4.2 & $13.5\pm0.4$\\
			& & 12.5 & $6.0\pm0.3$\\
			\hline
		\end{tabular}
		\label{tab:freqmasses}
		\caption{Table of the frequencies observed in our sample, in field regions where they are constant, below and above the metamagnetic transition.}
	\end{center}
\end{table}

%\begin{table}[t]
%	\begin{center}
%		\begin{tabular}[h]{|c|c|c|c|}
%			\hline
%			\multicolumn{2}{|c|}{5.5 to 6.5 T} & \multicolumn{2}{|c|}{9 to 12 T}\\
%			\hline
%			Peak (kT) & $m^*/m$ & Peak (kT) & $m^*/m$\\
%			\hline
%			0.15 & $3.0 \pm 0.1$ & 0.16 & $4.6 \pm 1.0$\\
%			0.45 & $6 \pm 1$ & &\\
%			0.9 & $6 \pm 1$ & 1.1 & $9 \pm 1$\\
%			& & 1.3 & $10.1 \pm 0.7$\\
%			1.8 & $6.8 \pm 0.3$ & 1.6 & $7.0 \pm 0.1$\\
%			2.8 & $3.8\pm0.5$ & &\\
%			3.0 & $2.5\pm0.1$ & 3.0 & $3.3\pm0.1$\\
%			& & 3.3 & $9.3\pm1.6$\\
%			& & 3.5 & $12\pm4$\\
%			4.2 & $9.5\pm0.3$ & 3.9 & $13.0\pm0.4$\\
%			& & 4.0 & $12.4\pm0.5$\\
%			& & 4.2 & $10\pm1$\\
%			& & 12.5 & $6.7\pm0.3$\\
%			\hline
%		\end{tabular}
%		\label{tab:freqmasses}
%		\caption{Table of the frequencies observed in our sample, in field regions where they are constant, below and above the metamagnetic transition.}
%	\end{center}
%\end{table}

Table \ref{tab:freqmasses} lists the observed frequencies and the associated masses, as found using a fit of the LK relation over the temperature dependent area under the peaks. Peaks are observed at the following frequencies: in the low field region, 0.15, 0.45, 0.9, 1.8, 2.8, 3.0 and 4.2 kT, and in the high field region, 0.13, 1.1, 1.4, 1.6, 3.0, 3.3, 4.0 (a split peak) and 12.5 kT.  In the previous work, it was suggested that the peaks seen at 0.15, 0.45, 1.8 and 4.2 kT evolve across the transition to become those at 0.13, 0.4, 1.6 and the split peak at 4.0 kT, respectively, and the one at 0.9 to the split peak at 1.1 and 1.3 kT. This is very clear at least for the 1.8 and 4.2 kT peaks, since the ones at 1.8 and 1.6 kT have a similar large amplitude and the ones at 4.2, 4.0 kT are very isolated. The peak at 1.8-1.6 kT is the dominant component of the signal in both field regions, and is mainly responsible for the shape of the oscillations seen in figure \ref{fig:1nHarmOsc}. Also, the quasiparticle masses agree well with values previously found, with lower error values. Finally, the peaks at 3.0 and 12.5 kT are associated, the calculated mass giving strong evidence, with the $\alpha$ and $\beta$ peaks of Sr$_2$RuO$_4$. The frequency of the 3.0 kT peak does not change as the system traverses the metamagnetic transition, unlike those of Sr$_3$Ru$_2$O$_7$. No trace was found of the $\gamma$ peak at 18.7 kT, but the presence of Sr$_2$RuO$_4$ was further demonstrated by the observation of superconductivity at low field, through the measurement of a diamagnetic signal in the susceptibility at low fields.

Figure \ref{fig: Frequencies} shows the field dependence of the frequencies of all the peaks observed in both field regions calculated with the windowing method (more details are given in the next section). The gaps in the curves indicate regions where the peaks are not resolved. The program used to calculate frequencies and masses decides by itself to keep or reject data in a given frequency interval of a given spectrum calculated for a specific field region, using a gaussian fit of the peak, based on a few simple assumptions: the center of the gaussian has to be inside the interval, the width of the peak has to be smaller than the interval, etc. The selection process was found to be very successful in filtering enormous amounts of data. 

To finish this section, at this point, let us make the remark that a few peaks are still not identified. Those are the 2.8 kT peak in the low field region and the 3.3 kT peak in the high field region. No trace of these frequencies was seen in the previous work although the peak at 4.2 kT, with a much lower amplitude, was detected, making it unlikely that they belong to \TTS. They don't seem related since their mass is very different. It is then clear from here that it would be highly desirable to use a single phase sample, without inclusions of other phases of the ruthenium oxide.

\begin{figure}[t]
\begin{center}
	\includegraphics[width=.80\columnwidth]{\PchapterIII Frequencies.eps}
	\caption{Frequency of all peaks seen in the second harmonic as function of field, calculated using the windowing method. The window size was 0.02 T$^{-1}$. Gaps or absence of data for these frequencies indicate regions where they are not detected.}
	\label{fig: Frequencies}
	\end{center}
\end{figure}

\subsection{Calculation of field dependencies near the quantum critical end point}

 \begin{figure}[p]
  \begin{center}
	\includegraphics[width=.80\columnwidth]{\PchapterIII 2kTFreqBoth.eps}
	\caption{Frequency of the 1.8 and 1.6 kT peak across the metamagnetic transition for first (triangles) and second (circles) harmonics.}
	\label{fig: 2kTFreqBoth}
	\end{center}
  \begin{center}
	\includegraphics[width=.80\columnwidth]{\PchapterIII 4kTFreqBoth.eps}
	\caption{Frequency of the 4.2 and 4.0 kT peak across the metamagnetic transition for first (triangles) and second (circles) harmonics.}
	\label{fig: 4kTFreqBoth}
	\end{center}
\end{figure}

 \begin{figure}[p]
  \begin{center}
	\includegraphics[width=.80\columnwidth]{\PchapterIII 1nHarmMass.eps}
	\caption{Mass ratio of the quasiparticle with respect to the electron mass, for the first harmonic.}
	\label{fig: 1nHarmMass}
	\end{center}
  \begin{center}
	\includegraphics[width=.80\columnwidth]{\PchapterIII 2nHarmMass.eps}
	\caption{Mass ratio of the quasiparticle with respect to the electron mass, for the second harmonic. The inset shows typical LK fits at different field windows.}
	\label{fig: 2nHarmMass}
	\end{center}
\end{figure}

We are interested in the field dependence of quasiparticle masses and frequencies in order to get insight into the physics involved as the system crosses the metamagnetic transition, the magnetic field being the tuning parameter for quantum criticality. As shown in sections \ref{sect:FFTwindowing}, \ref{sect:mass} and \ref{sect:envelope}, two methods can be used to calculate the field dependent mass, by windowing or envelope extraction, but the frequencies have to be determined with the windowing method. In order to obtain peaks of the same width, for a constant frequency, the same inverse field width for the windows has to be used for each data point, but they can overlap. If the frequency varies, then it is the same number of cycles of the specific oscillation we are looking at that is needed for each window. This is a very time and disk space consuming task, but when automated, very straightforward.

Figure \ref{fig: 2kTFreqBoth} and \ref{fig: 4kTFreqBoth} show the field dependence of the frequency for, respectively, the 1.8-1.6 and 4.2-4.0 kT peaks. There is a similar increase in both cases near the metamagnetic transition, and in both cases, the frequency is lower in the high field region than at low field, away from 7.8 T. This corresponds to a complex transformation of the Fermi surface structure. 

Figures \ref{fig: 1nHarmMass} and \ref{fig: 2nHarmMass} show field dependent masses of the 1.8-1.6 and 4.2-4.0 kT peaks, for both harmonics, calculated using the windowing method, with error bars. Gaps or discontinuities in the data indicate regions where the fit is either very bad, yields negative amplitudes or where the error is larger than the value. Causes for this problem are that either zero values of a beat pattern, large non-oscillatory features of the susceptibility or just poor signal to noise ratio. As one can observe, any divergence of the mass near 7.8 T is not at all obvious in this data, and we do not, at this point, reproduce the conclusion of the work by Borzi $et$ $al.$. 

This observation leads us to realise that there has possibly been a problem in these experiments with the thermometry in these experiments, producing a systematic error, making us calculate with a non-linear fit erroneous quasiparticle masses. The next section will address this issue.

\subsection{Avoiding eddy current heating in samples: parameter determination \label{sect:eddy}}

The effect of eddy current heating is to increase the sample temperature compared to that of the thermometer, which is located outside of the magnetic field region, at the mixing chamber. Even for small heating, the systematic error on the thermometry will have dramatic effects on the calculation of the quasiparticle effective masses. This can easily be understood when we consider that the effective mass is inversely proportional to the width at half maximum of the Lifshitz-Kosevitch temperature dependence (see figure \ref{fig: RLK}). A positive systematic error on the sample temperature will always make the non-linear fit of the Lifshitz-Kosevitch function underestimate the quasiparticle mass, and moreover, this effect will be more pronounced the higher the mass is. This can have the effect of suppressing, partly or completely, an enhancement of the quasiparticle masses described in the last section.

Consequently, one must determine if there is sample heating during an experiment in order to be able to trust any mass value. Since the source of heat is the rate of change of the magnetic field, one then has to use the lowest possible excitation field, but reducing this also reduces the amplitude of the signal, and a compromise has to be found. If the quasiparticle mass of one frequency is known, then measuring it as function of the amplitude or frequency of the AC field becomes a good measure of sample heating. The mass should saturate to a value as the excitation field decreases.

We saw in sections \ref{sect:plasticprobe} and \ref{sect:oscsignal} (see eq. \ref{eq:eddy} and \ref{eq:Mexpansion}) that, in the limit where $\lambda < 2$, 
\begin{enumerate}
\item Eddy current heating is proportional to $\dot{H}^2 \propto \omega^2 H_{AC}^2$,
\item The signal in the first harmonic is proportional to $\omega H_{AC}$,
\item The signal in the second harmonic is proportional to $\omega H_{AC}^2$ and is much smaller than that of the first,
\end{enumerate}
We can see from this that increasing by the same factor the AC field or its frequency produces the same increase in eddy current heating, as well as the same increase in signal in the first harmonic. However, with the second harmomnic, one gains in reducing the frequency while increasing the modulation field. 
Heating should be checked as function of modulation field amplitude and frequency. It is possible that in some cases, the second harmonic, even though measurable with very good signal to noise ratio at high AC field, cannot be measured without eddy current heating at all AC fields where it is above the noise. In that case, only the first harmonic should be used for mass analysis. However, if one is only concerned about dHvA frequencies, one should increase $\lambda$ to maximise $J_2(\lambda)$. Finally, when eddy current heating occurs, the adjusted quasiparticle mass will constitute a lower bound value for the real mass. One should check if discarding the lowest temperature data points enhances the value from the fit.

Figure \ref{fig: MassvsHacw} shows an analysis of eddy current heating in a sample of \TTS. DHvA was measured in a small magnetic field window where the signal is high, between 6.5 and 7.5 T, at five different temperatures, from 50 to 350 mK, at different modulation fields, from 1 to 16 G, at 15 Hz. The mass of the dHvA peak at 1.8 kT (the peak of highest amplitude) was calculated by fitting the LK relation, for all the AC fields used. We can see that when we include the lowest temperature data in the calculation, even though the fit is good, the value for the QP mass generated is significantly lower than when we exclude them. We conclude that heating is important at this temperature. 

\begin{figure}[t]
	\begin{minipage}[t]{7cm}
		\begin{center}
		\includegraphics[width=7cm]{\PchapterIII MassvsHacw50.eps}

		\end{center}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{7cm}
		\begin{center}
		\includegraphics[width=7cm]{\PchapterIII MassvsHacw100.eps}
		\end{center}
	\end{minipage}
	\caption{Non-linear fits of the LK relation for the 1.8 kT peak from first harmonic dHvA data generated with different modulation fields at temperatures between 50 and 350 mK, measured on a sample of \TTS, at a frequency of 15 Hz. The Fourier transforms were taken using field windows between 6.5 and 7.5 T. ($left$) Non-linear fits including the data points at 50 mK. ($right$) Non-linear fits excluding the data at 50 mK. One can see that for this system, a modulation amplitude of 4 G induces a tolerable error on the QP mass.}
	\label{fig: MassvsHacw}
\end{figure}



\newpage
%----------------------------------------------------------------------------------------------------------------

\section{AC susceptibility in an adiabatic demagnetisation refrigerator}


The de Haas van Alphen experiment, as we know from section \ref{sect:Impurities}, depends on the impurity scattering rate in an exponential manner. As we will explain in section \ref{sect:search}, obtaining a good sample is not trivial, but one such should improve dHvA data immensely compared to one of average quality. This means that a sample sorting procedure is needed. Moreover, preparing samples for the experimental apparatus described in section \ref{sect:plasticprobe} takes a long time, so that trying the dHvA experiment on many samples in this way would take too much time. Finally, the demand for the dilution refrigerator being very high, we needed an alternative solution for this task, which was to set up a new dHvA apparatus for the adiabatic demagnetisation refrigerator (ADR), for which there is much less demand, that can accommodate larger unprepared samples, and for which the running time from room to low temperature is shorter. 

Secondly, another possibility of interest was to detect superconductivity in \TTS samples, and this will be explained in details in section \ref{sect:superconductivity}. The detection of this phenomenon is most easily made using zero magnetic field AC susceptibility. Consequently, this new apparatus has two completely different uses that will prove to be necessary for this project.

This section describes the building, testing and use of this new experimental probe. It has become, with time, the second workhorse of this thesis project, as will be shown in section \ref{sect:dHvAADF}. Here, however, we will first describe the adiabatic demagnetisation refrigerator, then we will give the technical details of this AC susceptibility system and show the temperature tests that were made to it, and finally, we will show the first successful dHvA measurements that were carried out.

\subsection{The adiabatic demagnetisation refrigerator}


\begin{figure}[p]
	\begin{minipage}[t]{7cm}
		\begin{center}
		\includegraphics[width=7cm]{\PchapterIII ADF_1Ksketch.eps}

		\end{center}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{7cm}
		\begin{center}
		\includegraphics[width=7cm]{\PchapterIII ADF_LTSsketch.eps}
		\end{center}
	\end{minipage}
	\caption{Sketch of the ADR components. The left side of the figure shows the top part, featuring the 1-K pot stage, and the right side the low temperature stage (LTS). The whole system is located inside the inner vacuum chamber (IVC), in a vacuum of around 10$^{-8}$ mbar, which itself is submerged into liquid He$^4$, in a standard dewar, and slides into the bore of the demagnetisation magnet and the sample magnet. In normal operation, the 1-K stage is at a temperature of 1.6 K and is thermally connected to the heat shield that surrounds the LTS. It is cooled by the 1-K pot, by reducing the vapour pressure of He$^4$ using an external pump. Liquid He$^4$ is fed to the 1-K pot by the fill line, from the He bath in the dewar, outside the IVC. The LTS is thermally isolated from the 1-K stage by suspension with Kevlar strings, and connected to it using a mechanical heat switch. The LTS features the paramagnetic salt pill, which is used for adiabatic demagnetisation cooling, which is inside the bore of a 6.3 T superconducting magnet. The measurement apparatus, which can be, for example, an AC susceptibility system, a resistivity probe or a heat capacity measurement apparatus, is located in the sample space inside the 8 T superconducting sample magnet. The magnets are designed to cancel each other's magnetic field in a region between both, where is installed the thermometry, which can only function in a low field region. The LTS needs to be free of any contact with the heat shield, so that a centering mechanism that uses Kevlar strings is needed in the extreme lower part.}
	\label{fig:ADFsketch}
\end{figure}

The adiabatic demagnetisation refrigerator (ADR) is a very simple system. Its principle relies on the very high difference of entropy in a paramagnetic system between its states in high and low magnetic fields. The entropy is lowered by applying a high field, and then, when the system is put in thermal isolation, reducing the its amplitude will reduce the temperature by a transfer of entropy from the sample and measurement apparatus to the paramagnetic material.

Figure \ref{fig:ADFsketch} illustrates the main parts of the ADR system. It is put into a dewar filled with liquid He$^4$. The system features two important cooling mechanisms. The first is a standard 1-K pot, which cools the apparatus by pumping $He^4$ gas at the surface of liquid He$^4$, therefore lowering its vapour pressure and temperature, and is situated on the so called 1-K stage. It can be seen in the left half of the figure, which shows the top part of the apparatus. The first step of the adiabatic demagnetisation cooling process requires the user to cool the whole system to the 1-K pot temperature, which is of around 1.6 K, starting from liquid He boiling temperature at 1 bar, 4.2 K. 

The right side of the figure shows, on top, the paramagnetic salt pill, a cylinder of around 3 cm of diameter, 15 cm long, inside a 6.3 T superconducting magnet. This is the part which will produce adiabatic demagnetisation cooling. It is always put in the best thermal contact possible with the low temperature stage (LTS), the lower part of the ADR, where the measurement apparatus is located. The second step of adiabatic demagnetisation cooling consists in ramping the magnetic field of the demagnetisation magnet to 6.3 T, and wait for thermal equilibrium with the 1-K pot stage. The temperature normally increases during this process since we are effectively reducing the entropy of the paramagnetic salt pill to its lowest level, or in other words, expelling heat from it, and decreases again once the maximum field and thermal equilibrium are reached.

On the 1-K pot stage, in the left side of the figure \ref{fig:ADFsketch}, one can see the position of the heat switch. It is essentially an electrical contact switch, which is operated mechanically from outside the dewar. One can also see the Kevlar suspension thermal isolation, by which is hung the paramagnetic salt pill and the LTS below it. It has an extremely low thermal conductivity, making the lower part of the system in a quasi adiabatic state once the heat switch is opened. Carrying further the cooling process, once thermal equilibrium is reached between the 1-K pot stage and the paramagnetic salt pill, the user proceeds to the third step, which consists in opening the heat switch and gradually reducing the demagnetisation magnetic field. From this point, the LTS temperature will be approximately proportional to the magnetic field applied on the pill.

Finally, the LTS features two parts, the sample field region, which is within the sample field region, produced by an 8 T superconducting magnet, and the compensated field region, where the thermometry is located. The temperature is measured using two different thermometers, one for high and the other for low temperatures. For temperatures between room temperature and 1 K, we use a Cernox semiconductor resistive thermometer, and for temperatures between 1 K and 50 mK, the system automatically switches to a Ge semiconductor resistive thermometer. Next to these thermometers is also installed a resistive heater, that can be used to obtain temperatures higher than the 1-K pot temperature. The two magnets were designed such that the field amplitude is low in the compensated field region, in order to avoid magnetoresistive errors in the temperature measurements.

We will now derive a few equations describing the use of this type of refrigeration. As we already mentioned, the principle of adiabatic demagnetisation refrigeration uses the entropy of an isolated paramagnetic material and a magnetic field applied to it. Let us then look at a paramagnetic system. If the spins have a total angular momentum of $J = L + S$, their interaction with the field will be (see \cite{ashcroft} chapter 3)
\beq
\epsilon = -g(J,L,S)\mu_B\bs{J} \cdot \bs{H},
\eeq
with $g(J,L,S)$ the Landé factor. For a non-interacting system, the partition function for a single spin is
\bea
z &=& \sum_{states} e^{-{\epsilon \over k_bT}} = \sum_{k = -J}^J e^{-{kg\mu_B H \over k_B T}}\nn\\
&=& {e^{-{g\mu_B H \over k_B T}J}-e^{{g\mu_B H \over k_B T}(J+1)} \over 1-e^{{g\mu_B H \over k_B T}}} = {e^{-{g\mu_B H \over k_B T}(J+{1 \over 2})}-e^{{g\mu_B H \over k_B T}(J+{1\over 2})} \over e^{-{g\mu_B H \over 2k_B T}}-e^{{g\mu_B H \over 2k_B T}}}\nn\\
&=& {\sinh{g\mu_B H \over k_B T}(J+{1 \over 2}) \over \sinh{g\mu_B H \over 2k_B T}}.
\eea
The partition function for the whole system of $N$ spins will be
\beq
Z = {z^N \over N!},
\eeq
and the free energy $F$ is
\beq
F(H,T) = -k_BT \ln Z = -Nk_BT \ln{\sinh{g\mu_B H \over k_B T}(J+{1 \over 2}) \over \sinh{g\mu_B H \over 2k_B T}} + k_B T \ln N!.
\eeq
We can now obtain all the physical quantities we are interested in by differentiating $F$, for instance the magnetisation $M$ and the entropy $S$:
\bea
M = -\bigg({\partial F \over \partial H}\bigg)_T &=& N g\mu_B J B_J(gJx )\nn\\
S = -\bigg({\partial F \over \partial T}\bigg)_H &=& Nk_B\bigg[\ln{\sinh g(J+{1 \over 2})x \over \sinh{gx \over 2}} - gJxB_J(gJx)\bigg] - k_B\ln N!,\nn\\
\eea
with $B_J$ the Brillouin function,
\beq
B_J(y) = (1+{1\over 2J}) \coth(1+{1\over 2J})y - {1 \over 2 J} \coth {y \over 2 J}.
\eeq
The important point to make here is that both the entropy and the magnetisation are functions of $H$ and $T$ through $x = {\mu_BH \over k_BT}$ only, so that for an adiabatic process where $H$ varies, $T$ has to evolve such that the ratio $x$ remains constant. In such a scenario, by reducing $H$ to zero, the temperature would drop also to zero. It is not the case, of course, since below a certain field, $H_0$, the intrinsic internal field of the paramagnetic material becomes more important, and it depends on the strength of the very small but non-vanishing spin interactions. In other words, the spin system never reaches a state that is totally disordered due to spin interactions. When the system reaches the minimum field of $H_0$, the cooling power vanishes and we obtain a base temperature $T_{BT}$.

This analysis holds true when only the spin system is held in adiabatic conditions in the cryostat, or in other words, when no significant load of heat capacity is connected to it. In our system, we know that the heat capacity load is not negligible. It means that, as temperature is reduced, heat will be transferred from the LTS to the paramagnetic material, and the entropy of the spin system $S$ will not be constant anymore. Consequently, as we reduce the magnetic field, in a small step of $\Delta H$, the temperature reduces of $\Delta T$, but their ratio also changes by $\Delta x$, as does the entropy of the spin system by $\Delta S$, and 
\beq
- T\Delta S = C_M^{LTS}(T) \Delta T,
\label{eq:TdS_ADF}
\eeq
where $C_M^{LTS}$ is the heat capacity load of the LTS. $C_M^{LTS}$ corresponds in our case to a construction made mainly of copper, so we will assume it has the form of the heat capacity of a metal,
\beq
C_M^{LTS}(T) = N (\gamma T + \beta T^3),
\eeq
with $N$ the number of moles of copper. Let us define a path we will use during our demagnetisation process, where the rate of decrease of the temperature will be constant. We integrate eq. \ref{eq:TdS_ADF} over this path:
\beq
- \Delta S(T',H)  = \int_{T_{1K}}^{T} {C_M^{LTS}(T') \over T'} dT' = N (\gamma T + \beta {T^3\over 3}) + C,
\eeq
where C is a constant of integration. In order to observe the form of the implicit relation between $T$ and $H$, we need to produce a plot of the level curves of the total entropy, which is conserved,
\beq
N_s \Delta s +  N (\gamma T + \beta {T^3\over 3}) = C,
\eeq
where $N_s$ is the number of spins in the paramagnetic material in the pill and $\Delta s$ is a single spin's entropy, the expression of which we already have. In order to do so, of course, we need to determine the relative constants $N_s$ and $N$. Different operations on the system can be performed in order to measure these parameters, that are described in appendix ???. Results of this analysis are plotted in figure \ref{fig:HvsTcontour}. We see there an interesting fact, that is always observed during normal operation of the ADR, which is that the rate of decrease of the LTS temperature accelerates when one cools down the apparatus with a constant rate of demagnetisation, or, equivalently, the rate of demagnetisation slows down if one cools down using a constant rate of decrease of temperature. The reason for that is simply that the heat capacity of the whole LTS decreases with temperature faster than the cooling power does. One can then use any demagnetisation field profile, the system will always follow a level curve like in fig. \ref{fig:HvsTcontour}.

\begin{figure}[t]
\begin{center}
	\includegraphics[width=.7\columnwidth]{\PchapterIII HvsTcontour.eps}
	\caption{Contour lines of the total entropy of the LTS of the ADF while in adiabatic state, cooling down using a constant rate of decrease of temperature. The red lines correspond to high entropy, which decreases as the colour moves towards blue. The lines are effectively representing the implicit relation between the demagnetisation magnetic field applied on the paramagnetic salt pill and the temperature of the LTS. The path followed during operation will depend on the initial parameters, the starting magnetic field and temperature. The dashed line represents the intrinsic ordering magnetic field of the paramagnetic material, at which the cooling process will stop.}
	\label{fig:HvsTcontour}
	\end{center}
\end{figure}

In the limit of low heat capacity load, the entropy of the paramagnetic pill changes only very little while cooling down. We can make an approximation to eq. \ref{eq:TdS_ADF}:
\bea
-TdS &\simeq& T{dS \over dx}\bigg|_{x_0} dx =  N (\gamma T + \beta T^3)dT\nn\\
 x-x_0 &\simeq& {dS \over dx}\bigg|_{x_0}^{-1} N (\gamma T + {\beta \over 3} T^3 - \gamma T_0 - {\beta \over 3} T_0^3)\nn\\
H(T) &=& {H_0 \over T_0}T + {dS \over dx}\bigg|_{x_0}^{-1} N \big(- (\gamma T_0 + {\beta \over 3} T_0^3)T + \gamma T^2 + {\beta \over 3} T^4\big)
\eea
We see from this approximate equation for $H(T)$ that we should observe a linear behaviour with an added $T^3$ contribution at high temperatures, due to the phononic term of the heat capacity. The dominating term is the expected linear term of gradient ${H_0 \over T_0}$. In the limit of infinitely low heat capacity load, this linear term would be the only contribution and $x$ would be a constant, as we have already mentioned.

Finally, we should add some comments on the fact that the ADR system has a very small heat leak, which has to be taken into account when performing experiments. The heat transfer from the $He^4$ bath to the LTS takes place mainly through the Kevlar strings of the suspension and centring mechanisms, at the top and bottom of the LTS. The result of this is that the entropy will slowly increase such that the path followed when decreasing and increasing temperature will not be exactly the same, but it will still be very close to what we can see in fig. \ref{fig:HvsTcontour}. Also, when one wants to stabilise the temperature to a certain value, it will be possible by using a very slow almost constant demagnetisation rate, which will provide a cooling power equal to the heat leak,
\beq
\dot{Q} = T {dS \over dt} = T{\partial S \over \partial H}\bigg|_T \dot{H},
\eeq
and the system will move slowly horizontally towards the left in figure \ref{fig:HvsTcontour}.

%It will be proportional to the temperature difference between the LTS and the heat shield, which at the temperature of the 1-K pot, 
%\beq
%d\dot{Q} = K \nabla T,
%\eeq 
%where $K$ is the thermal conductivity. $K$ is not a constant at low temperatures, though, but rather has a temperature dependence from the phononic transport of heat, since Kevlar is an insulator. Such a thermal conductivity is proportional to $T^3$ (see, for instance, \cite{pobell} pp. 48-53), such that during the adiabatic cooling process, the entropy transferred to the LTS is
%\beq
%T dS_{leak} \propto T^3(T_{1K} - T) dt = -{1\over \dot{T}}T^3(T_{1K}-T)dT.
%\eeq
%When cooling down to temperature $T$, the total entropy contributed will be
%\beq
%\Delta S_{leak} \propto -{1\over \dot{T}}\int_{T{1K}}^{T} T'^2(T_{1K}-T')dT' = -{1\over \dot{T}}(T_{1K}{T^3\over 3} - {T^4 \over 4 }) + C
%\eeq

\subsection{AC susceptibility setup for large crystals}


Figure \ref{fig: ADFsuccprobeplan2} shows the schematics of the AC susceptibility probe for the ADF. It was designed to have as many pick-up coils as the space inside the refrigerator allowed, with a single modulation coil, as the ADF does not have one built-in. The pick-up coils were also made as large as was possible with still enough turns for them to be sensitive enough for our application, and this was in order to be able to measure the susceptibility of rough, unprepared chunks of crystal rods. 

Table \ref{tab:ADFCoils} lists all the parameters related to the coils. These were wound using copper wire, of 125$\mu$m for the drive coil and 50$\mu$m for the six pick-up coils, and the windings were glued using standard GE varnish. The leads of each of the coils are twisted closely together to avoid picking up noise when vibrating in the magnetic field, which are soldered to a 24 pin connector, into which the standard wiring of the cryostat can be connected. The pairing of the coils is made using one of two options, either outside the cryostat or inside, in this case using an adaptor that can be fitted between the probe connector and the cryostat wiring.

When using the adaptor to pair the coils inside the cryostat, one takes the advantage of using the three low temperature transformers that are fitted on the 1 K stage of the ADF, using an amplification factor of 100. This helps enormously to increase the signal to noise level of the measurement apparatus. With this configuration, noise levels between 100 pV/$\sqrt{\textrm{Hz}}$ and 1 nV/$\sqrt{\textrm{Hz}}$ (peak to peak) are generally obtained, if we take care of eliminating as much as possible acoustic noise and vibrations.

The samples are placed inside the pick-up coils by placing them inside a copper braid, which is inserted from the bottom of the apparatus (see figure \ref{fig: ADFsuccprobeplan2}), which is tightly screwed to the low temperature stage gold plated copper frame. The reason for using this is that the samples need to be very well thermally anchored in order for them to be in thermal equilibrium with the thermometry of the system. High vacuum grease is used to improve the thermal contact with the braid. We avoided using silver paint at this stage in order to still be able to clean them properly for the possibility of using them in various subsequent experiments. The thermal equilibrium of the samples with the system was verified, as will be shown in section \ref{sect:Tchecks}.

Finally, as explained in the last section, the total heat capacity of the measurement apparatus added to the low temperature stage of the ADF influences the base temperature one can reach, or equivalently, the length of time one can manage to stabilise the system to a certain temperature. This AC susceptometer is rather massive compared to the measurement probes that are generally installed on this system, so the lowest temperature we obtain is much higher than the base temperature quoted by the manufacturer, of 50 mK. We usually can reach between 100 mK and 150 mK, and it is possible to stabilise the temperature at 250 mK for around 100-150 minutes, which allows us to measure with sample field sweeps of 2-3 T of length at a rate of 0.02 T/min. It is quite difficult to stabilise the system at lower temperatures for any reasonable length of time.

\begin{figure}[p!]
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII ADFsuccprobeplan3.eps}
	\caption{Schematics of the AC susceptibility probe for the adiabatic demagnetisation refrigerator. All parts are made of tufnol (a plastic with good low temperature properties) or copper, except for the supporting stainless steel threaded rods. The primary coil has 2555 turns of 125$\mu$m copper wire, with a field to current conversion factor of 535 G/A. The odd shape of its top and bottom ends are designed to fit between the three support posts of the low temperature stage of the ADF. The central part holds six pick-up coils of around 800 turns each of 50$\mu$m copper wire. They are 3 mm long and separated by 4 mm. It slides inside the primary coil former from the top, and the samples are inserted from the bottom. The system is held together with three steel threaded rods and bolts. They keep in place the tufnol connector holder, into which is inserted a CMR 24 pin connector, secured with a side screw. Along two of the steel rods are inserted copper heat sink cylinders. The wire of the primary coil is wound around one of them, in the form of a twisted pair. The 12 wires of the six pick-up coils are wound around the second heat sink, where each pair of wires from each coil is carefully twisted in order to avoid the induction of noise in the wiring outside of the coils themselves. All the wires are soldered to the connector. Finally, the heat sinks are screwed tightly each to a copper braid, which will be put in good electrical contact with the low temperature stage of the ADF.}
	\label{fig: ADFsuccprobeplan2}
	\end{center}
\end{figure}



\begin{table}[p]
	\begin{center}
		\begin{tabular}[h]{|c|c c c c c |}
			\hline
			&&&&&\\
			Coil& Turns & Resistance & Resistance & Sensitivity & Offset (paired)\\ 
			&& $\Omega$ & (paired) $\Omega$ & $\mu$V/GHz & $\mu$V/GHz\\
			\hline
			1 & 794$\pm$5 & 133 && 10.37 &\\
			2 & 607$\pm$15 & 104 &  \raisebox{1.5ex}[0pt]{237}& 7.97 &  \raisebox{1.5ex}[0pt]{2.366}\\
			&&&&&\\
			3 & 790$\pm$5 & 136 && 11.33 &\\
			4 & 800$\pm$2 & 138 &  \raisebox{1.5ex}[0pt]{274}& 11.68 &  \raisebox{1.5ex}[0pt]{.3254}\\
			&&&&&\\
			5 & 802$\pm$2 & 137 && 11.57 &\\
			6 & 839$\pm$1 & 138 &  \raisebox{1.5ex}[0pt]{275}& 10.74 &  \raisebox{1.5ex}[0pt]{0.8225}\\
			&&&&&\\
			Drive & 2555 & 42 &\multicolumn{3}{c|}{535 G/A}\\
			\hline
		\end{tabular}
		\label{tab:ADFCoils}
		\caption{Technical data for the various coils of the AC susceptibility for the ADF. The coils of number 1 to 6 are the pick-up coils used for measurement, in order from the top to the bottom of the probe. The pairs 1,2; 3,4; 5,6 are connected in opposition. The table shows their number of turns and their resistance at room temperature for when they are both single or paired. This resistance reduces by a factor of around 100 at low temperature. The sensitivity refers to the voltage measured on one single coil when put in an oscillating magnetic field of one Gauss of amplitude at 1 Hz. When connected in opposition, if both coils of a pair are in the same field and empty, the voltage measured, shown in the last column, corresponds to the constant offset that will be measured on top of a magnetic signal during experiments. The last row contains the data related to the drive coil, used to create the modulation magnetic field. Its conversion factor from current to field was calculated using geometrical considerations.}
	\end{center}
\end{table}

\newpage
\subsection{Temperature checks using superconductors \label{sect:Tchecks}}

The new AC susceptibility experimental setup presented here is quite massive and involves a large former made of plastic. Since this plastic is insulating, it avoids eddy current heating, but it is also difficult to cool down below 1 K, so it was to be expected that it should act as a virtual heat leak at these low temperatures. The inconvenience with adiabatic demagnetisation is that the cooling power is finite, so that any heat leak determines not only the base temperature of the system, but also the time it can be kept at a constant temperature, while dHvA requires both low temperatures and very slow magnetic field sweeps. Moreover, the base temperature reached with the demagnetisation process depends directly on the total heat capacity of the low temperature stage. 

Any new low temperature experiment needs checks over whether the samples are at the same temperature as the thermometer, and we suspect here, due to the possible heat leak of the plastic, that the sample temperature might be higher than the measured temperature. The first step with this setup was then to measure a chosen physical phenomenon that arises at fixed temperatures, and the superconductivity transition of type one of different pure metals was chosen as ideal. The determination of a critical temperature $T_c$ is done by sweeping the temperature of the system while measuring the susceptibility at zero DC magnetic field. As shown in appendix \ref{App:C}, the transition appears as a discontinuous jump in the component of the measured voltage in phase with the modulation field, and as a peak in the component out of phase (components that are proportional to the in-phase and out of phase susceptibilities $\chi'$ and $\chi''$). The transition temperature is defined at the maximum of this peak.

There were two main concerns with this test. First, the transition temperature in pure metals is very sensitive to low magnetic fields ($H_c$ for the superconductors of type one we chose is of the order of 100 G). The superconducting magnet of the refrigerator has a remnant field, or flux trapped within its coil when it is superconducting, so that a constant magnetic field is always present, even when the magnet power supply is shut down. The magnet power supply of this system is not very accurate for low magnetic fields (below 100 G), and the solution was to use another current source and apply a current to the magnet that would cancel exactly the remnant field in the axial direction. Secondly, the shape of the sample must disrupt minimally the magnetic field lines in order that the field is constant over all parts of it, or in other words, the superconducting sample needs to have the smallest demagnetisation factor. The high purity material we used was in the form of 125 $\mu$m thick foil, so the ideal shape to use was that of a "swiss roll", a cylinder of rolled foil. Since the magnetic flux can penetrate the sample between the layers, the demagnetisation factor was minimised while the signal was still very easy to detect. 

The materials that were used are aluminium ($T_c = 1.196$ K, $H_c = 105$ G, \cite{kittel}), zinc ($T_c = 0.875$ K, $H_c = 53$, G \cite{kittel}), both of purity 99.999\%, and \TOF ($T_c$ = 1.5 K for the purest samples, $H_{c2} =$ 2 T, H $||$ $ab$-plane, 0.2 T, H $||$ $c$-axis, \cite{mackenzieRMP}) . Measurements were always taken with both decreasing and increasing temperature. The reason for that is that when any magnetic field is present, the superconducting transition is of first order and hysterisis appears as function of temperature (see \cite{pobell} pp 205-207). In other words, the transition arises at different temperatures when sweeping the temperature upwards or downwards. A magnetic field always shifts the downwards transition to lower temperature than the upwards transition, but moves both to $lower$ temperatures than the transition at zero magnetic field. The smaller the hysterisis, the closer the measured $T_c$ is to the real $T_c$. Since we expect the sample to be hotter than the thermometer and not colder, we should measure a transition temperature lower than the real $T_c$ even when there is no hysterisis. We should note here that we could only cancel the remnant field of the system magnet, but not any other like the earth's magnetic field ($\sim 0.5$G), so that the hysterisis could only be minimised. Moreover, there is no way to calculate what the remnant field of the magnet should be, and this latter actually changes when changing the current applied to the magnet. To cancel it, the current applied to the magnet was chosen such that the in-phase susceptibility was a minimum (the $T_c$ maximum) with the system at a temperature slightly lower than the expected transition temperature. 

Figure \ref{fig: PureAlZnCoils56-06} shows the results for Al and Zn obtained with the hysteresis minimised by cancelling the remnant field of the samples magnet. The data was taken using two different sweeping rates, upwards and downwards in temperature each time. We deduce transition temperatures from the highest of all four for each material, i.e. the slowest upwards sweep. We obtain 1.175 K for Al and 0.880 K for Zn. The real transition temperatures of 1.196 K and 0.875 K, respectively, yield an uncertainty of around 20 mK for our system in this temperature range. This is not extremely accurate, but the goal here was not to calibrate precisely the thermometry of this system, but rather to roughly verify it. We will see in the next section a more accurate way we have used to verify it again at lower temperatures.

Figure \ref{fig: Sr2RuO4Coils12-02} shows the susceptibility as function of temperature for small cubic samples of \TOF aligned with the $ab$ plane parallel and perpendicular to the magnetic field. We essentially obtain the same result, with critical temperatures of 1.53 K for H $||$ $ab$-plane and 1.55 K for H $||$ $c$-axis. The real value for the critical temperature is lower, 1.50 K, which is lower than what we measure, telling us at least that the samples, at this temperature, are not warmer than the thermometer.

Finally, it is also possible to roughly calibrate the voltages measured on the coils into real susceptibility values. For this, all one needs to do is to measure the change in voltage, as we sweep the temperature across the superconducting transition, when using a sample of superconductor for which we know well the demagnetisation factor. Figure \ref{fig: PureAlZnCoils56-06} tells us the amplitude of the diamagnetic signal of such a sample, with a demagnetisation factor that is very close to zero. Effectively, the shape that was chosen was of a cylinder of rolled Al foil. 
The voltage measured on a pair of compensated coils with such a sample placed into one of them will be
\beq
\Delta V = A R \dot{B} \chi,
\eeq
where $A$ is the total area enclosed by all the turns of the coil containing the sample and $R$ the fraction of this area intersecting the sample, which, if the turns are wound uniformly as in our case, will also be equal to the $volume$ fraction occupied by it, $R = v_{sample}/v_{coil}. We don't know $v_{coil}$, but we can find it from the sensitivity $S$ given in table \ref{tab:ADFCoils}. The voltage, with frequency $f$, measured on one empty coil is $V = A \dot{B} = S \dot{B} f$, so that the susceptibility will be given by
\beq
\chi = {\Delta V \over VR} = {\Delta V v_{coil}\over S \dot{B} v_{sample}}
\eeq
Using the voltage difference of 1.9 $mV$ from figure \ref{fig: PureAlZnCoils56-06}, which includes an amplification factor of 100, a frequency of 71 Hz, a field of 0.428 G, a mass of 52.6 mg and a density of 2.702 g/cm$^3$, we obtain a value for the volume of the coil of $v_{coil} = 0.3345 cm^3$. This can be used to simplify our equation to get, as a rough calibration of our coils
\beq
\chi = 3.1145\times10^4 ({cm^3 G Hz \over V}) {\Delta V \over B f v_{sample}}.
\eeq
Moreover, since we always use the values of $B = 0.428$ G, $f = 71$ Hz, an amplification factor of 100 and samples of density 6.117 g/cm$^3$ (for \TTS), we can rewrite if as
\beq
\chi = 62.7 (g/V) {\Delta V \over m_{sample}},
\eeq
where $m_{sample}$ is the mass of the sample.

%Using the amplitude of the excitation field $H_0$, its frequency $f$, the mass $m$ of the sample and the density $\rho$ of Al, we can obtain the conversion factor $C_{\chi}$, such that the susceptibility, which is equal $-1$, can be found from the voltage difference $\Delta V$ measured on the coils:
%\beq
%\chi = C_{\chi} {\Delta V \rho \over f H_0 m} = -1.
%\eeq
%Using the voltage difference of 1.9 $mV$ from figure \ref{fig: PureAlZnCoils56-06}, which includes an amplification factor of 100, a frequency of 71 Hz, a field of 0.428 G, a mass of 52.6 mg and a density of 2.702 g/cm$^3$, we obtain a value for $C_{\chi}$ of -89.2 G Hz cm$^3$/V. This value is valid for coil 6 (see table \ref{tab:ADFCoils}), but all the other coils have sensitivities that vary by at most 3\% (except for coil 2, but it is usually used as a compensation coil).

In order to verify the validity of this calculation, we can take the parameters that we know characterise the coils and try to reproduce the value of -89.2 G Hz cm$^3$/V. Table \ref{tab:ADFCoils} tells us the voltage we should measure on coil 6, with a modulation field of 1 G at a frequency of 1 Hz, if a superconductor filled completely the space inside its windings, from the sensitivity value of 10.74$\mu$V/GHz. The volume to use in this calculation is not obvious, since there are several layers of windings, so that they don't all have the same inner area. Using a weighed average value for the area inside a winding of 0.275 cm$^2$, we obtain a volume of 0.0825 cm$^3$. Dividing the volume by the sensitivity, we obtain a value for $C_{\chi}$ of -83.4 G Hz cm$^3$/V. It is not quite the same value, and the error is obviously due to the estimated volume inside the coil, but it is close enough to convince us that the value of -89.2 G Hz cm$^3$/V is valid.

\begin{figure}[p]
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII PureAlZnCoils56-06-Al.eps}
	\end{center}
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII PureAlZnCoils56-06-Zn.eps}
	\caption{In-phase and out of phase susceptibility as function of temperature for swiss roll shaped samples of high purity aluminium and zinc (99.999\%) with the hysteresis minimised. The data was taken using two different sweeping rates, 0.11 K/min and 0.04 K/min, upwards and downwards in temperature each time.}
	\label{fig: PureAlZnCoils56-06}
	\end{center}
\end{figure}

\begin{figure}[p]
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII Sr2RuO4Coils12-02-c.eps}
	\end{center}
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII Sr2RuO4Coils12-02-ab.eps}
	\caption{Susceptibility as function of temperature for samples of \TOF, one oriented with  H $||$ $c$-axis (top) and the other with  H $||$ $ab$-plane (bottom).}
	\label{fig: Sr2RuO4Coils12-02}
	\end{center}
\end{figure}

\newpage

\subsection{The de Haas van Alphen experiment in the adiabatic demagnetisation refrigerator \label{sect:dHvAADR}}

The first step towards the goal of detecting quantum oscillations in arbitrary samples is to measure them in with a known material. For that, we used a sample of some of the best quality ever made \TOF. The dHvA analysis was made in a more than complete fashion in the past \cite{bergemann}. Three oscillation frequencies were reported, at 3.05, 12.7 and 18.5 kT, the first one with an amplitude overwhelmingly larger than that of the others. Consequently, our first objective was to detect the oscillations at this frequency. 

\begin{figure}[p]
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII Sr2RuO4Coils12-03.eps}
	\end{center}
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII Sr2RuO4Coils12-03-FFT.eps}
	\caption{Oscillations of the in-phase magnetic susceptibility as function of magnetic field (top) for a sample of \TOF. The spectrum of the Fourier transform of these yield an extremely well defined peak at 3.0 kT (bottom). No other frequencies were detected. Integrating the peak in the power spectrum, taking the square root and dividing by the mass of the crystal and the amplification factor of 100, we obtain approximately 5 $\mu$V/g of signal amplitude.}
	\label{fig: Sr2RuO4Coils12-03}
	\end{center}
\end{figure}

Figure \ref{fig: Sr2RuO4Coils12-03} shows the first successful result, that it is in principle possible to measure quantum oscillations in our apparatus. The top part shows the oscillations observed in $\chi'$, while the bottom part shows the FFT spectrum of these, where a peak is found at 3.0 kT. By integrating the peak in the power spectrum of the FFT and dividing by the mass of the crystal and the amplification factor of 100, we obtain a value for the oscillation amplitude of about 5 $\mu$ V / g. 

We later want to use this system for sorting samples of \TTS. The current average purity of this material being nowhere near that of our \TOF sample, and the Dingle factor driving the purity dependence of the dHvA amplitude exponentially, we generally obtain values for the amplitude per mass much lower, in the few tens of nV/g. Figure \ref{fig: Sr3Ru2O7C697A} shows typical data measured on \TTS. The integrated amplitude measured in this case is of about 50 nV/g, 100 times smaller than the value obtained for \TOF.

There are checks that can be made on such dHvA data taken over short field ranges in order to demonstrate its authenticity. Some oscillatory noise periodical in time can sometimes appear as a peak in an FFT taken as function of inverse field. These usually dissapear when the data set is taken over a large field range, since the noise is not periodical as function of inverse field. In order to differentiate the two, the best criterium to use is the phase. The phase of dHvA should always be the same at a same magnetic field value in multiple measurements, but not the noise. Moreover, one can check if the oscillations have a temperature dependence, and once again, the phase of the measurements does not change with temperature.

\begin{figure}[p]
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII Ltr2Ltr3-dHvA-02a.eps}
	\end{center}
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII Ltr2Ltr3-dHvA-02a-FFT.eps}
	\caption{Oscillations of the in-phase magnetic susceptibility as function of magnetic field (top) for a typical sample of \TTS among the large number that were analysed in the sorting procedure demonstrated in section \ref{sect:search}. The bottom graph shows the FFT spectrum, where a peak is found at 1.8 kT. The integral of this peak yields an amplitude value of about 50 nV/g.}
	\label{fig: Sr3Ru2O7C697A}
	\end{center}
\end{figure}

Finally, one last rough check on the thermometry can be made using the quantum oscillations. It consists in measuring an already known quasiparticle mass of one of the dHvA frequencies. We of course took the same frequency of 1.8 kT and measured the oscillation amplitude as function of temperature, between again 6 and 7 T. The integrated amplitude is shown in figure \ref{fig:MassRunC698A}, with a LK fit. The value for the quasiparticle mass of this frequency reported by Borzi $et. al.$ \cite{borzi} is of $m^*/m = 8 \pm 1$. We calculated, with a slightly more accurate fit, a value of $m^*/m = 8.4 \pm .1$, in accordance with the reported value. As we saw with eddy current heating into samples in section \ref{sect:eddy}, a positive systematic error on the sample temperature will make the LK fit underestimate the quasiparticle mass. Therefore, since our value is $higher$ than the reported value, and we know that  Borzi $et al.$ were very careful with their own temperature measurements, we conclude that our thermometry in this experiment is accurate enough for our purposes. Note that, as can be seen in \cite{borzi}, the quasiparticle mass is still constant in the field region between 6 and 7 T, but increases with higher fields. 

\begin{figure}[t]
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII MassRunC698A.eps}
	\caption{dHvA integrated amplitude of the 1.8 kT frequency as function of temperature for a sample of \TTS. The stars are the data, and the solid line is a LK fit. The quasiparticle mass extracted by the fit is of $m^*/m = 8.4 \pm .1$. The previously reported value was of $8 \pm 1$ \cite{borzi}.}
	\label{fig:MassRunC698A}
	\end{center}
\end{figure}


\newpage
\section{Systematic procedure for the search for ultimately pure samples \label{sect:search}}

\begin{figure}[ht]
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII SampleRoad1.eps}
	\caption{Standard recipe for cutting the crystal rods grown in the image furnace for the various experiments in the sorting procedure. The rods are cut into slices of 1.8 mm thick. These are then further cut to obtain a square prism around 3 mm long. These parts are the samples and will be kept for the susceptibility and magnetisation experiments. The off-cuts will be used for measuring the residual resistivity and the X-ray spectrum. The residual resistivity and the X-ray spectrum of the square prism is assumed to be the same as that of the off-cuts, and agree only approximately with the other measurements. Note that the $ab$ axes can have any orientation within the $ab$-plane.}
	\label{fig: SampleRoad1}
	\end{center}
\end{figure}
 
As was described in the introduction for this chapter, the purity requirements for the de Haas van Alphen experiment are very high. For this work, I was lucky enough that I could interact with the the materials scientist that was growing the crystals of \TTS, R.S. Perry, since this was done in the laboratory next door. The strategy was one of feedback style, where I carried out a chain of characterisation methods on grown samples and provided the information back to R. S. Perry, in order for him to improve the growth parameters and restart the process. The sample sorting procedure was carried out using two types of characterisation methods. First, we will describe those used to detect different phases of ruthenates. Second, we will talk about the determination of sample purity.

In early de Haas van Alphen experiments, we have used an average quality sample of \TTS. We obtained relatively good quantum oscillations data, but we had to use a very high modulation field in order to obtain a good signal to noise ratio, which led to eddy current sample heating, an effect we came to understand later. This sample also led us to erroneous interpretations when we discovered a dHvA frequency at 12.7 kT, that belongs to \TOF. It became clear that the sample was not purely of the bilayer type but had small inclusions of \TOF. This would lead us to suspect that it might also contain some \FTT and \OOT, etc. Moreover, these inclusions of \TOF clearly had a purity comparable to that of the \TTS, since we detected the oscillations well. Consequently, any good sample for dHvA should be thoroughly checked for all possible foreign phases before its oscillation spectrum can be interpreted. 

We used the magnetic properties of the different phases of the ruthenate to identify them quantitatively. The reason for that is that only \TTS is paramagnetic at all temperatures. The $n=\infty$ (\OOT) and $n>3$, (\FTT, etc) members of the Ruddlesden-Popper series are ferromagnetic with Curie temperatures below room temperature \cite{Cao,Crawford,Cao2, Kanbayasi}. We also expect the phases with $n > 3$ to be ferromagnetic, but no evidence of their presence was observed. We used a Superconducting Quantum Interference Device (SQUID) magnetometer at small fields for detecting the spontaneous ferromagnetic moment of our samples. And finally, as we already know, the $n=1$ phase, \TOF, is a superconductor with a transition temperature of 1.5K or less (for complete information on \TOF, see \cite{mackenzieRMP}). We used AC susceptibility at zero field to detect the diamagnetic behaviour of the samples. 

The next subsections will describe all the characterisations that we applied to our samples, in the order that they were used. The order is important for saving a lot of time. The first and quicker methods determine if the samples are good enough to be submitted to the next. The first experiment to be performed on a newly grown crystal rod is powder X-ray diffraction, which identifies all the crystalline components of the material, but which is also destructive. It is performed with a small piece of crystal that will be ground to a fine powder, and the content of the rod will have to be assumed from that result. The second experiment is to measure the resistivity as function of temperature, where one chooses a long and thin plate of crystal and mounts it in the way that will be described. When we extrapolate it absolute zero, we obtain a value proportional to the disorder in the crystal. Again, the disorder in the larger crystal rod will have to be assumed from this value. Next, the samples that seem promising are put into the AC susceptibility system of the ADR, for the next two experiments. Crystal rods that have good properties will be divided into as many samples as possible. With the AC susceptibility, we will measure the diamagnetic content of the sample, and with dHvA, the disorder. And finally, the ferromagnetic content of the samples will be measured with the SQUID magnetometer.

This procedure was performed on over 50 samples from around 10 crystal rods. 24 of them have made it through the five experiments and were kept for this project. Figure \ref{fig: SampleRoad1} illustrates the way the crystal rods are divided for the various experiments. The sample that we used in the early stages of this thesis project into extensive dHvA analysis was used as a standard with which to compare. The last subsection will present a summary of the data taken on these samples. We will demonstrate later that the X-ray spectra and the residual resistivities agree only approximately with the other measurements, although they are still good starting points. 
 

\subsection{Powder X-ray diffraction}

\begin{figure}[h]
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII Xrays.eps}
	\caption{Example of powder X-ray measurements. The top spectrum is of a crystal containing some detectable \TOF and \FTT intergrowths, while the bottom one is pure enough that these phases are not seen in these measurements. The top curve was offset for clarity. Most of the peaks belong, as we expect, to \TTS, and appear at angles of 8.6$^{\circ}$, 17.2$^{\circ}$, 23.3$^{\circ}$, 31.6$^{\circ}$ and 32.6$^{\circ}$. There is only one peak one can easily recognise for \TOF, at 13.9$^{\circ}$ in this angle interval. There are two peaks for \FTT, at 12.4$^{\circ}$ and 18.6$^{\circ}$, but the latter one has the highest intensity. No peak allows us to easily identify \OOT, as they are all too close to peaks that belong to \TTS. The angle interval is chosen for clarity; the higher angles are populated with too many peaks produced by \TTS.}
	\label{fig:Xrays}
	\end{center}
\end{figure}

The first and easiest measurement that is performed on all the new crystal growths is the powder X-ray spectrum. It takes half an hour to perform and tells us of the various phases of strontium ruthenate that are present into the new crystal. This method is of course destructive, so it is carried out on a small amount of single crystal crushed to powder, and the result has to be assumed to extend to the rest of the crystal. As we will see in the next sections, this is true in a very approximate manner. Nevertheless, this measurement is always done in order to ascertain that the main phase produced during crystal growth is actually \TTS.

The measurement is produced with a copper X-ray source, that emits at a wavelength of 1.54 \AA, and a CCD camera that detects the reflection intensity of the rays as function of angle. The various atomic planes of the crystal will reflect the X-rays at specific angles, which are tabulated in standard databases. Figure \ref{fig:Xrays} shows two examples of spectra, one featuring only Bragg peaks associated with \TTS, and the other one exhibiting additional peaks, of \TOF and \FTT. The chosen angle range is between 5$^{\circ}$ and 35$^{\circ}$. The reason behind this choice is that the higher angles are populated with much more peaks from bragg planes of \TTS, such that identifying other phases becomes difficult. The main peaks that belong to \TTS between 5$^{\circ}$ and 35$^{\circ}$ are located at 8.6$^{\circ}$, 17.2$^{\circ}$, 23.3$^{\circ}$, 31.6$^{\circ}$ and 32.6$^{\circ}$. When these are present, \TOF has only one peak which is easily distinguished from the others, at 13.9$^{\circ}$, and \FTT has two, at 12.4$^{\circ}$ and 18.6$^{\circ}$, the second with a higher amplitude. Unfortunately, \OOT features peaks that are too close to those of \TTS or not intense enough to be used for its identification. In most cases, we know from magnetisation experiments that \OOT is present in small amounts, but none of the X-ray peaks of this phase are observed. Figure \ref{fig: Xrays} displays two powder X-ray measurements, one of which featuring only peaks that are produced by atomic planes of \TTS, and the other possessing a few more peaks, that belong to \TOF and \FTT.

Since each X-ray spectrum features an arbitrary intensity factor, only amplitude ratios between various peak intensities are meaningful. Consequently, when measuring the amount of \TOF or \FTT with this method, we take the ratio $R$, in the first case, of the peak at 8.6$^{\circ}$ of \TTS with that of the one at 13.9$^{\circ}$ of \TOF, and in the second case, the peak at 8.6$^{\circ}$ again with the peak at 8.6$^{\circ}$ of \FTT. These ratios yield values greater than zero in a normal case where the main phase present is \TTS. Note that in the 22 samples that we kept for the experiments, only one featured a content of \FTT detectable with powder X-ray diffraction, C6102A, which is the one shown in figure \ref{fig:Xrays}. It thus means that all our samples contain relatively small amounts of this type of intergrowths.

\subsection{Resistivity and residual resistivity}

\begin{figure}[ht]
	\begin{minipage}[t]{9cm}
		\begin{center}
		\includegraphics[width=9cm]{\PchapterIII RRsample1.eps}

		\end{center}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{4.5cm}
		\begin{center}
		\includegraphics[width=4.5cm]{\PchapterIII rho_Res.eps}
		\end{center}
	\end{minipage}
	\caption{$Left$ Illustration of a mounted resistivity sample in a four point resistivity measurement configuration. The sample is oriented with the $ab$-plane in the horizontal direction. Its size is typically of around 1 mm long, .1 mm wide and .01 mm thick. Two voltages are measured, in order to verify the uniformity of the sample, and reject the possibility of a $c$-axis contribution. The sample is mounted on a quartz substrate and is elevated such that it is not in contact with it. The 50 $\mu m$ thick wires holding it in mid-air are made of gold and are fixed with high temperature cured silver epoxy, shown in light gray. One must make sure that all the contacts are attached with silver paint to the whole thickness of the sample, such that the current does not travel in the vertical direction inside the sample. $Right$ Typical measurement of the resistivity as function of temperature, with a fit of expression \ref{eq:residualres}. The low temperature region follows a $T^2$ behaviour, while the intermediate region is linear in $T$. The extrapolation of the $T^2$ fitted expression to absolute zero yields the residual resistivity $\rho_0$.}
	\label{fig:RRSample1}
\end{figure}

The standard method to determine disorder in a sample is to measure its residual resistivity, in the $ab$-plane direction (the $ab$-plane being the direction in which \TTS cleaves easily, this is the easiest configuration to use). As was discussed in section \ref{sect:FermiLiquid} (??? more specific), in a highly correlated metal, the resistivity as function of temperature at low temperatures can be expressed as 
\beq
\rho(T) = \rho_0 + AT^2,
\label{eq:residualres}
\eeq
where higher powers of $T$ are neglected. The $T^2$ term is fundamental to the Fermi liquid theory, with the parameter $A$ depending on parameters of the metallic state like the quasiparticle mass $m^2$ and the Fermi wave vector $k_F$. Here, we are interested in the constant $\rho_0$, which depends only on static lattice disorder,
\beq
\rho_0 = {m_e\Gamma_0 \over ne},
\eeq
with $m_e$ the bare electron mass, $n$ the density of carriers and $\Gamma_0$ the scattering rate of the electrons due to lattice imperfections and impurities. It is standard to measure disorder in units of $\mu\Omega cm$, and one simply needs to fit the expression for $\rho(T)$ given here, extrapolating the data to absolute zero. Experience tells us that in our measurement apparatuses, \TTS samples that feature a $\rho_0$ of $1 \mu\Omega cm$ or less are likely to exhibit quantum oscillations, and those with a residual resistivity higher than that are not. The best known \TTS samples had $\rho_0 \simeq 0.3 \mu\Omega cm$.

An illustration of a sample mounted in a four point $ab$-plane resistivity measurement configuration is given in the left side of figure \ref{fig:RRSample1}. A very thin crystal is first cleaved off from a larger one, and then mounted on a quartz substrate such that it is held in mid-air by thin gold wires. In order to obtain a good signal to noise ratio, the sample geometry needs a very high aspect ratio. Its typical dimensions are of 1 mm $\times$ 0.1 mm $\times$ 0.01 mm. Six contacts are used such that two resistivity measurement are made per sample, one on each side of the crystal. The quality of the electrical contacts is determined by comparing these two measurements, which should be identical. The most common problem that arises is that of a $c$-axis contribution to the resistivity, where bad quality electrical contacts at the current leads forces the current to travel in the $c$-axis direction, for which the resistivity tensor component is around 300 times higher at 0.3 K than its $a$-axis or $b$-axis components \cite{Ikeda2000}, and leads to erroneous residual resistivities.

The measurements are performed in a simple liquid He flow cryostat. This system can  reach temperatures between room temperature and slightly below the boiling temperature of liquid He at atmospheric pressure, 4.2 K. For \TTS, this base temperature is low enough in order to obtain a reasonable amount of data in the $T^2$ dependence region of $\rho(T)$ that enables us to extrapolate it to absolute zero. The measured resistance is converted to resistivity using the known value at room temperature of 232 $\mu \Omega cm$. The right side of figure \ref{fig:RRSample1} shows a typical resistivity measurement and $T^2$ extrapolation. 

\subsection{Zero field AC susceptibility \label{sect:superconductivity}}

\begin{figure}[h]
\begin{center}
	\includegraphics[width=0.8\columnwidth]{\PchapterIII ACsuscC698I.eps}
	\caption{Typical zero field AC susceptibility measurement. The top curve (red) is proportional to the out-of-phase susceptibility $\chi ''$, while the lower one (blue) is proportional to the in-phase susceptibility $\chi '$. The data was divided by the mass of the sample in order to obtain a mass measurement. The peak in $\chi ''$ gives us the critical temperature for the metal to superconductor transition, while the amplitude of the diamagnetic signal, the value at which $\chi '$ saturates towards low temperature, is, to first order, proportional to the superconducting mass fraction of the sample. The arrows indicate the direction of the temperature variation: it was first lowered from 1.6 K to .1 K, and then raised again to 1.6 K.}
	\label{fig: ACsuscC698I}
	\end{center}
\end{figure}

The most sensitive method to determine the presence of the superconducting phase \TOF in samples that we intend to use for dHvA experiments is to measure the AC susceptibility at zero magnetic field, as function of temperature below 2K. As we saw in figure \ref{fig: Sr2RuO4Coils12-02}, the transition from the metallic state to superconductivity is observed by a jump in the in-phase AC susceptibility ($\chi '$) and a peak in the out-of-phase AC susceptibility ($\chi ''$). In the limit where the demagnetisation factor of these inclusions is near one, the amplitude of the jump in $\chi '$ is proportional to the volume of superconducting material. If we divide this by the sample mass, it will be proportional to the mass fraction of the sample that is \TOF.

The measurements are done with the opportunity that it is made in the same apparatus as for the dHvA experiments of the next section, and consequently, with the same cooldown of the refrigerator. It also implies that the samples are positioned with their $c$-axis parallel to the axis of the coils, as is required for dHvA. We expect, and know from polarised light optical microscopy experiments done by Fittipaldi $et$ $al.$ \cite{fittipaldi}, that the \TOF inclusions have a geometry that is of flat islands perpendicular to the $c$-axis, with the $c$-axis of the \TOF in the same direction as for the \TTS. Therefore, this geometry will make our calculation of the superconducting fraction difficult, but we will still assume that the diamagnetic signal is proportional to it in a first order approximation. 

The parameters of these experiments are the following. The magnetic field is set to zero, which means that only a remnant field is present of less than 50 G. The temperature is swept from the 1-K pot temperature to the base temperature and back to the 1-K pot temperature of the ADR at a rate of 25 mK/min. Finally, the samples are excited with a modulation field of 0.428 G at a frequency of 71 Hz.

In order to estimate the volume fraction from the amplitude of the diamagnetic signal measured in the $c$-axis direction, some assumption has to be made about the demagnetisation factor $n$. We will suppose the following: the average demagnetisation factor in the $c$-axis direction is approximately the same in all samples, or in other words, the shape of the inclusions has a distribution that is statistically the same. This is reasonable for samples that contain small amounts of \TOF, according to the polarised light experiments. The second assumption we will take is that the demagnetisation factor in the $ab$-plane direction is $n=0$, such that in that direction we would measure the real susceptibility, and hence the real volume fraction. Using these affirmations, by measuring the AC susceptibility of only one sample in the $ab$-plane direction should provide us with an approximate proportionality factor for all the other samples. 

We measured the AC susceptibility in both directions of Sample 2005, which yielded similar curves as the one shown in figure \ref{fig: ACsuscC698I}, but with an amplitude of 0.011 V/g in the $c$-axis direction, and ???? V/g in the $ab$-plane direction. The ratio of the first to the second minus one will give us the demagnetisation factor, $n = $????. Using the normalisation factor of section \ref{sect:Tchecks} of $C_{\chi}$ = 98.2 G Hz cm$^3$/V,  the density of \TTS, $\rho$ = 6.117 g/cm$^3$ and the demagnetisation factor $n$, we can convert the measured values for all samples, in V/g, into absolute susceptibilities:
\beq
\chi = {\Delta V \rho C_{\chi}\over m (1+n)},
\eeq
which should range between 0 and -1. This corresponds effectively to a fraction of the real susceptibility of a sample that would be entirely superconducting, and consequently to the volume fraction of \TOF into \TTS.


\subsection{de Haas van Alphen \label{sect:dHvAADF}}

\begin{figure}[ht]
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII dHvA+FFT_C698I.eps}
	\caption{Typical dHvA measurement performed in the ADR. The top curves, with axes at the right and top, feature the oscillations in the measured voltage, which is proportional to the in-phase susceptibility. The lower curve is the absolute value of the Fourier spectrum, with axes at the left and bottom. The integral of the peak at 1.8 kT in the spectrum divided by the sample masses yields an intensity for the oscillations of 100 nV/g in this case, the mass being of 80 mg.}
	\label{fig:dHvA+FFT_C698I}
	\end{center}
\end{figure}

The best way to determine in a comparative way the disorder in large crystals of high quality is to perform a dHvA experiment on them. Using our new AC susceptibility system described in section \ref{sect:dHvAADR}, we systematically measure samples with the same parameters such that the amplitude of dHvA is comparable between different samples. In order to be able to compare the quality of the various samples, one takes the square root of the integral of the power spectrum, divided by the mass. We generally obtain values between zero and 100 nV/g, this last value being the highest we have recorded. Note that these values are always measured with the $c$-axis parallel to the magnetic field, which we know from previous measurements, yields the highest oscillation amplitude.

Intensity values of 10 nV/g are usually close to the noise levels of our susceptibility system. These generally range from 100 pV/$\sqrt{Hz}$ to 2 nV/$\sqrt{Hz}$. Since we always use a time constant for detection of one second, transformers with amplification factors of 100 and sample masses of about 50 mg, this corresponds to intensities between .5 and 10 nV/g. When only noise is observed we mark the intensity value with a $less$ $than$ symbol but still quote the integrated intensity in the usual frequency region.

The parameters used for measurement are the following. We apply a modulation field of 0.428 G at a frequency of 71 Hz. We use the field region between 6 and 7 T, where, for \TTS, the oscillations have the highest amplitude, and vary the DC field at a rate of 20 mT/min. We verified carefully that these parameters don't cause eddy current heating, as was described in section \ref{sect:Tchecks} (see, in particular, figure \ref{fig:MassRunC698A}).

\subsection{Magnetisation}

\begin{figure}[p]
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII SquidExample2.eps}
	\caption{Magnetisation measurements performed with the SQUID magnetometer. $Left$ Hysterisis loops measured on sample C6102A, which features high amounts of \OOT and \FTT. The top graph is for a measurement with the magnetic field along the $c$-axis, and the bottom one for the $ab$-plane. In the $c$-axis case, both ferromagnetic materials become saturated below 1T and are indistinguishable. Hysterisis can be observed around zero field. When the magnetic field is in the $ab$-plane, three super-linear increases are observed, around 0, 2.5 and 4 T, with the first two featuring hysterisis. The increase at zero field is associated with \OOT \cite{Cao2}, while the one at 2.5 T is produced by \FTT \cite{Cao}, and that near 4 T is from \TTS \cite{perry1}. $Top$ $right$ Typical SQUID mass susceptibility measurements as function of temperature, with the sample field cooled at a magnetic field of 20 G. The dashed curve is for a very pure sample of \TTS, while the solid one was measured on a sample featuring small amounts of \OOT and \FTT. Three signals are superimposed, the paramagnetic signal of \TTS, which possesses a peak at around 16 K and the ferromagnetic transitions of \OOT and \FTT. $Bottom$ $right$ Field cooled mass susceptibility as function of temperature for sample C6102A, with a magnetic field of 20 G. The ferromagnetic signals of \OOT and \FTT are large enough to cover completely the paramagnetic signal of \TTS. Using their amplitude extrapolated to 0 K, and the total masses of \OOT and \FTT calculated using saturated ferromagnetic moments shown in figure \ref{fig:FerroSignal0K}, this type of measurement can be calibrated in order to get the fraction of the mass composed of these two materials.}
	\label{fig:SquidExample2}
	\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
	\includegraphics[width=.8\columnwidth]{\PchapterIII FerroSignal0K.eps}
	\caption{Values of the extrapolation to 0 K of the field cooled spontaneous magnetisation performed at various magnetic fields. The squares are for \OOT and the circles for \FTT. Both sets of data are symmetric, indicating that the remnant field of the SQUID magnet is very small. Moreover, they saturate towards 0.1 T.}
	\label{fig:FerroSignal0K}
	\end{center}
\end{figure}

Measuring the magnetisation offers the easiest way, in our laboratory, to detect ferromagnetic signals in samples with extremely high sensitivity. We had the opportunity to use a Quantum Design MPMS Superconducting Quantum Interference Device magnetometer (SQUID). This system can reach temperatures between room temperature and 2 K, and fields of up to 5 T. It allows, among other things, to measure the DC magnetisation as function of temperature or magnetic field

When measuring on our samples the magnetisation as function of temperature, starting at room temperature and decreasing to 5 K, at small fields, we generally observe two super-linear rises of the total magnetic moment, at around 100 K and 160 K (see figure \ref{fig:SquidExample2}, top right). The first is the Curie point of \FTT \cite{Cao} and the second, that of \OOT \cite{Cao2}. These are superimposed on the paramagnetic signal of \TTS, which is well known and features a peak at 16 K \cite{Ikeda2000}. This paramagnetic moment is smallest at low fields, where it is generally smaller than the ferromagnetic spontaneous moment of \OOT and \FTT when these impurity phases are present, even in very small quantities. It is thus very easy in this way to detect quantitatively their presence, and for that we only need to calibrate the amplitude of the two ferromagnetic signals into mass fractions of our samples. Figure \ref{fig:SquidExample2}, bottom right, shows the field cooled spontaneous magnetisation of sample C6102A, the one that exhibited the most intense  ferromagnetic signals. They are three orders of magnitude higher than the paramagnetic signal of \TTS at this field value.

To further demonstrate the presence of ferromagnetic materials in our samples, one must perform hysteresis loops. The left side of figure \ref{fig:SquidExample2} shows hysterisis loops performed on sample C6102A, for magnetic fields aligned with the $c$-axis (top) and the $ab$-plane (bottom). In the first case, the ferromagnetic signal for both materials are indistinguishable and saturate below 1T, indicating that the easy axis of \OOT is probably not in the same direction as that of \FTT, but rather lies in the direction of the bilayer of \TTS. In the second case, it is \FTT, as we know \cite{Cao}, that features hysterisis loops that are not centred at zero field, making its identification easy. We see three sharp rises in magnetic moment, at 0, 2.5 and 4 T. They correspond, in order, to \OOT \cite{Cao2}, \FTT and \TTS, \cite{perry1}. The first two feature hysteresis, but not the third one, as we would expect for two ferromagnetic and one paramagnetic materials. 

In order to calibrate our measurement of the field cooled spontaneous magnetisation as function of temperature for all our samples, we will use sample C6102A, for which we can neglect the presence of \TTS in such experiments, making our calculations easier. We want to determine the mass of each ferromagnetic impurity phase. With a simple fit of power laws, it is easy to extrapolate to zero temperature the total moment of each ferromagnetic phase. Figure \ref{fig:FerroSignal0K} shows how these moments evolve with the magnetic field at which the samples are cooled, for both \OOT and \FTT. We can see that the data is symmetric, and that it is saturated above 0.1 T. Using these saturated moments of 0.112 emu (\OOT) and 0.180 emu (\FTT), and those given by Cao (\cite{Cao,Cao2}) of respectively approximately 1.0 $\mu_B$/Ru and 1.1 $\mu_B$/Ru, which converted gives 23.6 emu/g and 22.7 emu/g, we obtain total masses of 4.7 mg of \OOT and 7.9 mg of \FTT. These correspond to 9\% and 16\% of the total mass, and we expect that none of the other samples should contain more of these phases.

Let us look once more at the lower right graph of figure \ref{fig:SquidExample2}. The total magnetic moment values extrapolated to 0K, when not normalised by the sample mass and the magnetic field, are of 0.049 emu (\OOT) and 0.075 emu (\FTT). With the masses previously calculated, we get the values of magnetic moment at 20 G of 12.9 emu/g and 10.3 emu/g, which constitutes our calibration.

Finally, we will use a similar fit with power laws for all the field cooled magnetisation data that we measure on the other samples, although, for some of them, the paramagnetic signal will be comparable to the ferromagnetism, so that this contribution will have to be substracted. Nevertheless, it is fairly easy to obtain extrapolations to 0K of the magnetic moments, and these values, when divided by the values that we calculated, will yield the approximate mass fractions we are looking for.


\subsection{Complete quantitative results of the search}

\begin{table}[p]
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII 327Samples1.eps}
	\caption{Complete quantative results of all characterisation methods for all the samples that were analysed. The two columns after the first give the integrated dHvA amplitude for the 1.8 kT peak, related to \TTS, and the 3.0 kT peak, related to \TOF. The fifth column is the ratio R of the powder diffraction peaks at 13.9$^{\circ}$, associated with \TOF, and 8.6$^{\circ}$, of \TTS. The higher R, the lower the amount of \TOF inclusions. The next two show the residual resistivities measured on each side of each resistivity crystals. Next come the columns with data from AC susceptibility, the first of which giving the superconducting critical temperatures, and the second the amplitude of the diamagnetic signal. Finally, in the last two columns we have the amplitude of the ferromagnetic signals of \OOT and \FTT measured with the SQUID. The first row of data belongs to the sample that was used in the preliminary experiments of section \ref{sect:preliminary}, and will be the standard with which to compare all the measured physical properties. The empty elements of the table indicate measurements that were impossible for various technical reasons.}
	\label{tab:327Samples1}
	\end{center}
\end{table}

\begin{table}[p]
\begin{center}
	\includegraphics[width=1\columnwidth]{\PchapterIII 327Samples2.eps}
	\caption{Fractional mass of the impurity phases \TOF, \OOT and \FTT in ppm, for all the measured samples. These are quoted along with the amplitude values of dHvA and the average residual resistivity, for convenience. Five samples feature remarkable dHvA properties. Among them, one possesses by far a much higher dHvA signal, C698I, while one contains negligible amounts of the impurity phases, C698A. Sample C698H contains no detectable trace of \OOT and \FTT, while it contains an amount of \TOF that is not negligible. The combination of the properties of these three samples is good enough to be able to rule out any dHvA signal that belong to the impurity phases in further high resolution extensive dHvA experiments.}
	\label{tab:327Samples2}
	\end{center}
\end{table}

In this section, we will present the complete results of the sorting procedure for samples of \TTS. Table \ref{tab:327Samples1} holds together all the measured quantities using all the characterisation methods described in this section: powder X-ray diffraction, residual resistivity, dHvA, zero field AC susceptibility and low field magnetisation. Some results are very good, and we will explain why. The same measurements were performed on the sample that was used in the preliminary experiments of section \ref{sect:preliminary}, denoted here, with the first row of data, "Sample 2005", for comparison purposes.

Using the various calculations described in the previous sections, one can obtain fractional values for the amount of inclusions of \TOF, \OOT and \FTT in each sample. Table \ref{tab:327Samples2} summarises these values, along with the same amplitude values for dHvA as the previous table, and the average residual resistivity, for clarity. Reading carefully this table should reveal the strategy to employ when choosing which samples to choose for extensive dHvA experiments.

The very first column of interest is that of the amplitude of the quantum oscillations at 1.8 kT. Sample 2005 gives us a value for comparison: all samples with a value higher than 16.5 nV/g are worth using in dHvA experiments, as they will yield more intense signal, but six of them have exceptional values, which are C697C, C698A, C698B, C698F, C698H and C698I. As we know from experience with crystal growth, it is hardly surprising that most of them should come from the same growth experiment, C698. According to these data, sample C698I features by far the highest amplitude, 100 nV/g, over 6.5 times that of Sample 2005.

The next column of interest is that of the mass fraction of \TOF calculated from the amplitude of the superconducting diamagnetic signal. We can observe that even within a single crystal batch, for instance C698, the amount of \TOF varies by orders of magnitude. Among our samples of interest, it is sample C698A that features the smallest amount of such inclusions, 50 times less than Sample 2005. It is also of interest to find that the highest value belongs to Sample 2005, meaning that in this respect, all samples are cleaner that this one. Moreover, the sample which is best for dHvA, C698I, features a lot more \TOF than C698A, by a factor 38.

The third set of values to look at is that of the mass fraction of \OOT and \FTT, calculated from the magnetisation. The two values, for each sample, seem correlated in an obscure manner. In reality, this is not surprising. Intuitively, we know that these inclusions correspond to stacking faults in the material. The $n > 2$ members of the Ruddlesden-Popper series are supposed to have physical properties that resemble more and more to that of the $n = \infty$ member as $n$ increases, such that it is probable that slight deviations in the growth parameters can produce a whole variety of them, and members with very large $n$ are essentially indistinguishable from $n = \infty$. However, the fractional values for \OOT and \FTT are visibly not correlated with those for \TOF. The sample with the smallest amounts of \OOT and \FTT is C698H, for which the ferromagnetic signals were not at all observed. In this regard, Sample 2005 contains very small amounts of these, while for sample C698I the fractions are 4 (\OOT) and 39 (\FTT) times larger. Sample C698A also contains very small amounts of ferromagnetic inclusions, which are barely detectable.

Finally, one can look at the column with residual resistivity data. It is very surprisingly not correlated with the column for dHvA. This effect can only be explained by the fact that the resistivity crystals are not representative of the dHvA ones, much less of the whole crystal rod, at least at these levels of purity. One can only rely on residual resistivity to infer disorder in a crystal rod on a much larger scale of values, where quantum oscillation experiments are not possible.

Before we finish this section, we will make a few more observations. Let us look at the data from the powder X-ray experiment, in table \ref{tab:327Samples1}, which, once more, has no correlation with the amplitude of the diamagnetic signal produced by \TOF. As for residual resistivity, they are not representative of large crystals, except to insure that \TOF is not actually the main phase produced by the growth experiment. A signal is almost $always$ observed at 13.9$^{\circ}$, even in cases where very low amounts are present in neighbouring regions. Also, in some instances, the quantum oscillation signal of the 3.0 kT orbit of \TOF can be observed, and its amplitude is not correlated with that of the diamagnetic signal. Since in such cases, the quality of the inclusions has to be very good, the disorder in \TOF intergrowths is not correlated with the fractional amount. However, the correlation can probably be made between the amplitude of the signal of the 3.0 kT dHvA frequency and the superconducting critical temperature, as was demonstrated by Mackenzie $et$ $al.$ \cite{PRLMackenzie}.

In conclusion, we will summarise with the strategy we have followed for the extensive dHvA analysis of \TTS that is at the core of this thesis project. In order to maximise the dHvA signal, there is no doubt about which sample to use: it should be C698I. But we know now, from our preliminary experiments (section \ref{sect:preliminary}) and our sorting procedure, that it is possible that when using the dHvA system for the dilution refrigerator, which has a much higher resolution than the one for the ADF, that we observe in that sample dHvA frequencies that are produced by either \TOF, \OOT or \FTT. dHvA was performed for the first of these in details, but the data for the other two in the litterature is not convincing enough to rely on in order to identify them. Moreover, these frequencies might actually cover features that belong to \TTS. Consequently, we will have to use also samples with slightly higher disorder levels but lower amounts of the foreign phases, samples C698A and C698H, in order to make sure that we don't make any interpretation error related to the other phases of the ruthenates.







